Leveraging Historical Associations between Requirements and Source Code to Identify Impacted Classes

As new requirements are introduced and implemented in a software system, developers must identify the set of source code classes which need to be changed. Therefore, past effort has focused on predicting the set of classes impacted by a requirement. In this paper, we introduce and evaluate a new type of information based on the intuition that the set of requirements which are associated with historical changes to a specific class are likely to exhibit semantic similarity to new requirements which impact that class. This new Requirements to Requirements Set (R2RS) family of metrics captures the semantic similarity between a new requirement and the set of existing requirements previously associated with a class. The aim of this paper is to present and evaluate the usefulness of R2RS metrics in predicting the set of classes impacted by a requirement. We consider 18 different R2RS metrics by combining six natural language processing techniques to measure the semantic similarity among texts (e.g., VSM) and three distribution scores to compute overall similarity (e.g., average among similarity scores). We evaluate if R2RS is useful for predicting impacted classes in combination and against four other families of metrics that are based upon temporal locality of changes, direct similarity to code, complexity metrics, and code smells. Our evaluation features five classifiers and 78 releases belonging to four large open-source projects, which result in over 700,000 candidate impacted classes. Experimental results show that leveraging R2RS information increases the accuracy of predicting impacted classes practically by an average of more than 60% across the various classifiers and projects.

==> Approach2.tex <==
\section{Approach}
\label{sec:Approach}
Our approach trains a classifier to predict whether an individual class will be impacted by the new requirement using a combination of Object-Oriented coupling and complexity metrics, change history, and text analysis. In this section we describe the various factors that we considered and the intuitions that led to their inclusion in CCP. Building the class predictor encompasses a four step process. 
\setdefaultleftmargin{30pt}{}{}{}{}{}
\begin{itemize}
    \item [Step 1]{{\bf Code and requirements linkage}. Requirements are linked to commits and the first commit per release is recorded.}% and serialize the results. During this step, we also extract the commit number of each release.}
    \item [Step 2]{{\bf Metrics measurement}. All metrics are computed for each commit, with the exception of temporal locality which is measured once at the first commit of each revision level. This is due to the high computational resources required by the approach.}
    \item [Step 3]{{\bf Metrics aggregation}. All metrics data is formatted into an ARFF file for use in training the WEKA classifier.}
    \item [Step 4]{{\bf Prediction and evaluation}. Finally the WEKA classifier is trained to predict the set of classes impacted by a new requirement. The predictor is evaluated for accuracy.}
\end{itemize}
Each of these steps are now described in greater detail.
\setdefaultleftmargin{12pt}{0pt}{0pt}{0pt}{0pt}{0pt}

\begin{figure}[!t]
	\begin{center}
		\includegraphics[width=.48\textwidth]{Overview2.pdf}
		\caption{Overview of our Class Change Predictor (CCP). Metrics are computed using a combination of static code analysis, requirements similarity scores, and change history.}
		\label{fig:Overview}
	\end{center}
\end{figure}

\subsection{Code and Requirements Linkage}
The first step in the process involves identifying explicit, user-defined, links between requirements and code. To accomplish this task we assume that developers include the ID of the relevant requirement in the source code commit message. For example, if a requirement is created named TIKA-11, the commit associated with the requirement must have TIKA-11 in its commit message. Assuming the project is named TIKA, the commit is evaluated with the regular expression: $.*TIKA-([0-9]+).*$. This is a reasonable assumption and is in fact assumed by Jira's own plugin for connecting to GitHub. As a result we identify a set of commits associated with each requirement, a list of files that were touched by those commits, and an approximate list of untouched files present in the system at the time of the commit. This list is approximate because developers may not have consistently tagged each commit message with the relevant requirement.  Finally, we identify the set of requirements associated with each class. We refer to this as the class's \emph{Requirement Set}. Furthermore, if the set contained more than ten requirements we retained only the ten most recently associated ones. 

\subsection{Metrics Measurement}
%JCH: Bunch of text moved to "parkingLot.tex" for now
Our CCP prediction model utilizes a diverse set of metrics to capture characteristics of the source code, requirements, and their interelationships over time.  In this section we describe each of these metrics in detail.

\subsubsection{Requirements to Class Associations}
One of the fundamental assumptions of CCP is that semantically similar requirements are likely to impact a similar set of classes. \vspace{4pt}\\
\noindent$\bullet$~{\bf Requirement-to-Requirement Similarity} CCP therefore needs to compute the similarity between each pair of requirements in a system. We evaluated several different algorithms for computing similarity. First, a series of standard pre-processing steps were used to prepare the text \cite{jivani2011comparative}.  These included removing non alpha-numeric characters, splitting CamelCase class, method, and variable names (e.g. camel case), and stemming each word to its morphological root using the Porter stemmer  \cite{jivani2011comparative}. The similarity between two requirements was then computed using several different Term Distribution based methods, i.e. Vector Space Model and Jensen Shannon Divergence, and Semantic Similarity based method including Optimum Comparator, Corley Mihalcea Comparator, and Bleu Comparator. A brief description of each approach is provided in Table X. \hilight{Jin?? See Justin's Thesis sec 2.1.3}. Each technique produces a score representing the similarity between each pair of requirements
.\vspace{8pt}\\
\noindent$\bullet$~{\bf Requirement to Class-Set Similarity}
The initial CCP Step used the Github commit messages to identify the  \emph{Requirements Set} associated with each class. When a new requirement is introduced, CCP computes the similarity of that requirement with each existing requirement (as previously described), and then uses the individual similarity scores to compute the similarity between a new requirement $R$ and the set of requirements associated with each class in the following ways:

\begin{itemize}
\item {\bf Maximum}: The computed score represents the highest individual similarity score between $R$ and the class's Requirement Set.
\item{\bf Median}: The median similarity score is used.
\item{\bf Average of Top Five:} The five most similar requirements are selected and their similarity scores averaged.
\end{itemize}

Considering all combinations of requirements similarity algorithms and class associations resulted in 18 (i.e. 6 $\times$ 3) additional candidate factors used to train the the source code impact predictor
.\vspace{12pt}\\
\noindent$\bullet$~{\bf Direct Requirement-to-Class Similarity}
In addition to computing the similarity between a new requirement and a class's Requirement Set, we also calculate the direct similarity between the new requirement and the textual content of the source code. Developers often using meaningful names for classes, methods, and variables, and also comment the code, this textual content can be used to estimate the similarity between a requirement and a class (REFS). Because the text in the source code is typically not in the form of complete sentences, CCP computes requirements to code similarity using only Term Distribution based methods (i.e. Vector Space Model and Jensen Shannon Divergence).  These requirements-to-class similarity scores are included as factors in the CCP classifier.

\subsubsection{Temporal Locality}
Each requirement in a class' requirement set has one or more time stamp associated with it representing the position(s) in the sequence of commits at which the requirement impacted the class. Several prior studies have shown that classes that have been frequently modified in the past are more likely to be impacted by future changes (REFS), and furthermore that recent changes are more impactful than older changes. We therefore computed the following three scores as a means of representing the potential impact that a requirement has on the current state of a class. 

\noindent$\bullet$~{\bf Simple Count:\%} \\ This divides the number of times the class had been touched up until that point in the history by the total number of commits in which that class existed. 
\begin{equation} 
{k}/{n} 
\end{equation}

The next two factors take into consideration \emph{temporal locality}. Kim et al. pioneered the use of temporal locality in predicting software changes, building a variety of caches to weight the importance of prior software modifications \cite{kim2007predicting}. Bernstein et al. rolled up the number of modifications for a class by month for the most 6 recent months, and used those temporal features to train a defect-predicting classifier\cite{bernstein2007improving}. With both of these concepts of temporal locality in mind, we computed temporal locality of recent modifications in three different ways for each class.

In the following formulas, $k$ is the number of modifications for the class as well as the index of the oldest modification. $N$ is the total number of commits involving the class, whether it was touched or untouched. $I$ is the number of the current modification, with the most recent commit involving the class having index 1. The closer the modification is to index 1, the most recent modification, the more weight it will be given.\vspace{4pt}\\

\noindent$\bullet$~{\bf Linear}
This approach applies more weight to recent class modifications. Given that the most recent commit index is 1, the modification of the class at commit index 2 will be given a weight of .5, the modification at index 3 will be given the weight 1/3, etc. All of these weights are divided by the total number of commits from the creation of the class until the current point in time.
\begin{equation}
\frac {\sum_{i=1}^{k} \frac{1}{i}}{n} \
\end{equation}

\noindent$\bullet$~{\bf Logarithmic} \\
Using a linear locality may assign insufficient weight to older modifications. In this approach we divide by $ln(k)$ when k is greater or equal to 3, allowing the weight to locality more gradually. 
\begin{equation}
\frac {\sum_{i=1}^{k} \frac{1}{ln(i)}}{n} \
\end{equation}
For example, a modification at commit index 4 will be given a weight of $1 / ln(4)$, the modification at commit index 5 will be given a weight of $1 / ln(5)$.  All weights are again divided by the total number of commits from the creation of the class until the current point in time. The differences in locality rates are illustrated in Table \ref{tab:locality} - which shows requirements 1, 3, 4, 8, and 9. 


\begin{table}[]
\centering
\setlength{\tabcolsep}{3pt}
\caption{Example of Temporal Locality Result for three classes}
\label{tab:TemporalLocalityTable}
\begin{tabular}{|c||c|c|c|c|c|c||c|c|c|}
\hline
Class & \multicolumn{6}{c||}{Requirement Touch} & \multicolumn{3}{c|}{Temporal Locality Results} \\ \cline{2-10} 
Name & 1 & 2 & 3 & 4 & 5 & 6 & Simple & Linear & Logarithmic \\ \hline
A & X & X & X & X & 0 & 0 & \textbf{0.67} & 0.16 & \textbf{0.47} \\ \hline
B & 0 & 0 & X & X & X & 0 & 0.5 & 0.18 & 0.44 \\ \hline
C & 0 & 0 & 0 & 0 & X & X & 0.33 & \textbf{0.25} & 0.33 \\ \hline
\end{tabular}
\end{table}

To better understand the calculation of temporal locality scores, it is useful to map out a simple example. Given Table \ref{tab:TemporalLocalityTable}, six different requirements have been implemented, impacting three different classes. 
For the \emph{simple} calculation, we see that class A has been touched four different times producing a score of $\approx$ 0.67 (i.e. 4/6). Class B has been touched three times, and there are a total of six requirements, so the modification score is 0.5, while Class C has a score of $\approx$ 0.33. 

The linear approach teakes temporal locality of the class modification into consideration. Class A has been touched at its sixth oldest modification, so we add one sixth to our running total. Class A was also modified at its fifth-most, fourth-most, and third-most recent commits, so we add that all to the running total, divide by 6, to produce a score of .16. Class B has more recent modifications, but less total modifications, but we can see that it still has a higher score at .18 than class A does.  Class C has the least total modifications with only 2, but it has the highest linear temporal locality score at .25. This exemplifies how heavily the linear temporal locality method favors recent modifications.

The logarithmic calculation works very similarly to the linear calculation, but we can see that it penalizes older activity substantially less than the linear method. We find that the logarithmic scores are just under the simple frequency calculations, as the penalty for older modifications is very slight.

All three history scores are included in the data used to train the classifier.

\subsubsection{Static Code Analysis}
While complexity metrics are typically used to identify refactoring opportunities and to predict bugs, we included several OO complexity metrics in our model based on the notion that complex and tightly coupled classes are more likely to be impacted by changes -- whether those changes directly or indirectly impact the class.  The following metrics were selected as being broadly representative (more?)\vspace{4pt}\\
\noindent $\bullet$~{\bf Code Smells}
The Sonarqube java plugin used in this project comes with over 1000 rules setup \cite{sonarsource2013sonarqube} including a number related to bad-smells such as \textit{private methods that do not access instance data should be static}, performance related, such as \textit{``wait(...)'' should be used instead of ``Thread. sleep(...)'' when a lock is held}, and security related, such as \textit{``public static'' fields should be constant}. We expect that if a class violates several of these rules, it is likely to need refactoring, and thus more likely to be changed. For each class file in a release, we measure the number of code quality rule violations.\vspace{4pt}\\

In addition we evaluate additional metrics which measure the coupling, cohesion, size, and complexity of each class using the metrics defined in Table X.

begin{table}[]
\centering
\setlength{\tabcolsep}{3pt}
\caption{Source Code Coupling, Cohesion, and Complexity Metrics}
\label{tab:CodeMetrics}
\begin{tabular}{|c|c|c|}
	\hline
	Metric&Tool&Description\\ \hline
	Code Violations&SonarQube&Defines rules for detecting code smells.  The metric counts the number of code smell violations. (Error Propensity)\\ \hline
	KeyWord Count&SonarQube&Counts number of key-words (e.g. if, else, for, while, etc. (Size, Complexity)\\ \hline
	LOC: Lines of Code&CKJM&Counts number of lines of code (excluding white space and brackets).   (Size)\\ \hline
	WMC: Weighted Methods per Class&CKJM&Sums number of methods per class, weighted by the cyclomatic complexity for each method.  (Size, Complexity)\\ \hline
	DIT: Depth of Inheritance Tree &CKJM&Measures the number of levels in a class's inheritance tree. DIT is an indicator of code-reuse. (Coupling)\\ \hline
	NOC: Number of Children&CKJM&Measures the number of times a class has been subclassed.  (Coupling)\\ \hline
	CBO: Coupling between Object Classes&CKJM&Measures the number of non-inheritance based associations to other classes.  (Coupling)\\ \hline
	RFC: Response for a Class&CKJM&Counts the methods that may be invoked by a class in response to an event.  (Coupling)\\ \hline
	LCOM: Lack of Cohesion of Metrics&CKJM&Measures the extent to which methods in a class are internally cohesive.  (Cohesion)\\ \hline
	Ca: Afferent Couplings&CKJM&Measures the number of direct references from other classes. (Coupling)\\ \hline
	NPM: Number of Public Methods&CKJM&Measures the number of publicly exposed methods. (Cohesion, Coupling)\\ \hline
	\end{tabular}
\end{table}


\noindent$\bullet$~{\bf  Code Complexity}
\hilight{Logic of refactoring doesn't fit this paper}
Code complexity in Sonarqube is a simple measure of the number of key-words (if, else, for, while, etc.) used in a code fragment \cite{sonarsource2013sonarqube}.
        
We expect that the more complex a class file is, the more likely it will be to need refactoring. We thus take a measure of the code quality for each class in a release. \vspace{4pt}\\
\noindent$\bullet$~{\bf Lines of Code}
We expect that larger class files are more likely to be in need of refactoring. We measure the number of lines of code (excluding white space and curly braces) for each class file in each release.\vspace{4pt}\\
%\noindent$\bullet$~{\bf Change Frequency}
%The change history metric is simply a class's number of past touches divided by its total touch opportunities. We expect that in many software projects, class files changed in the past are likely to be changed again in the future.\vspace{4pt}\\
%\noindent$\bullet$~{\bf Linear Temporal Locality}
%We expect that in many code-bases, classes that have been modified more recently are more likely to change in the future. We employ linear temporal locality scores, which heavily weight more recent changes to class files, to each class based on recent modification history.\vspace{4pt}\\
%\noindent$\bullet$~{\bf Logarithmic Temporal Locality}
%Logarithmic temporal locality, like the linear variety, weights recent modifications more than "stale" modifications. However, it penalizes "stale" modifications much less than the linear metric. We expect that the logarithmic metric will be an effective balance between the previous two approaches. \vspace{4pt}\\
\subsubsubsection{CKJM}
\hilight{can someone introduce CKJM?}
\noindent$\bullet$~{\bf CKJM WMC: Weighted methods per class}
The WMC is the sum of the cyclocomatic complexities for each method in a class \cite{cho2001component}. If a class has 3 methods, with method foo having a complexity of 3, method bar having a complexity of 5, and method fizz having a complexity of 2, the WMC of the class will be 10. We expect that classes with complex methods are more likely to be refactored.\vspace{4pt}\\
\noindent$\bullet$~{\bfDIT: Depth of Inheritance Tree}
The DIT measures the number of levels in a class's inheritance tree. If one class extends another class in Java, the child class will possess the methods of the parent class. Thus, the DIT measure shows how much code re-use a class has \cite{cho2001component}. We expect that classes with higher DIT scores are less likely to be refactored. \vspace{4pt}\\
\noindent$\bullet$~{\bf NOC: Number of Children}
The NOC score measures the number of times a given class has been sub-classed. Sometimes in industry, a class can be implemented with poor abstraction, and its children need to make many custom member variables as a result, leading to more total sub-classes in the project \cite{cho2001component}. It is our hypothesis that classes with higher NOC scores are likely in need of refactoring, and thus more likely to be modified by the user.\vspace{4pt}\\
\noindent$\bullet$~{\bf CBO: Coupling between object classes}
For each class-file, CBO measures the number of non-inheritance related connections to other classes. Classes with a high CBO measure are generally much harder to modify, as modifications to the class in question can affect many other class files \cite{cho2001component}. We expect that classes with high CBO are likely in need of refactoring, and thus more likely to be modified. \vspace{4pt}\\
\noindent$\bullet$~{\bf RFC: Response for a Class}
The RFC is the count of all methods that can be invoked by a class in response to user input. A high RFC score is indicative of a class that will be difficult for developers to understand, and thus more time-consuming to modify. We expect that classes with high RFC scores are likely in need of refactoring, and thus more likely to be modified.\vspace{4pt}\\
\noindent$\bullet$~{\bf LCOM: Lack of cohesion in methods}
The LCOM score is used to measure the level of cohesion of methods in a class. If a class has many methods that operate on the same instance variables, it will have high cohesion. If a class has multiple methods that have no instance variables in common, it will have low cohesion \cite{cho2001component}. We expect that classes with low LCOM scores are likely in need of refactoring, and thus more likely to be modified.\vspace{4pt}\\
\noindent$\bullet$~{\bf Ca: Afferent couplings}
 For a given class, its afferent coupling score measures the amount of times that other classes in the project reference the given class. Classes with high afferent coupling scores are usually more difficult to modify, as sometimes many other coupled classes will need to be modified along with it \cite{cho2001component}.  We expect that classes with high afferent coupling scores are likely in need of refactoring, and thus more likely to be modified.\vspace{4pt}\\
\noindent$\bullet$~{\bf NPM: Number of public methods}
NPM in java measures the number of methods that have been exposed as public. Classes with many public methods can sometimes have poor cohesion, given that any accessing class can call the class's methods \cite{cho2001component}. We expect that classes with low LCOM scores are likely in need of refactoring, and thus more likely to be modified.

==> Classifier.tex <==
\subsection{Metrics Aggregation}
Once all metrics have been measured, they are aggregated into a profile which is then used to train and evaluate the CCP classifier. Each row in the profile represents the measures for a requirement-class pair. The first two columns specify the requirement ID and the class name. The next 33 columns represent the metrics computed for the requirement-class pair as described in Section \ref{sec:Metrics}. Finally, the last column depicts whether the requirement impacted the class i.e. was explicitly linked to the class via a commit message. We generated an ARFF file from this profile to serve as an input to WEKA for evaluating CCP.

\subsection{Prediction and Evaluation}
\label{sec:Prediction}
Once the data is assembled to be used by the predictor, CCP performs three substeps, each detailed in a specific subsection below. 
 

\subsubsection{Pre-processing via PCA}
\label{sec:PCA}
Because individual metrics may be highly correlated, it can be useful to preprocess them using a method such as PCA which reduces dimensionality of the features \cite{jolliffe2002principal}. PCA has been extensively used in the software engineering domain \cite{briand2000exploring, falessi2013empirical, Nagappan:2006bugsprediction}. PCA bears similarities to the process of Singular Value Decomposition in linear algebra. If we consider a matrix, $M$, which is an $N \times P$ matrix with N values and P variables (or features), we can construct a diagonal variable matrix by taking $V=M^TM/(n-1)$ \cite{jolliffe2002principal}. The eigenvectors for this data are called the principal directions, and projections onto this space are called the principal components or dimensions \cite{jolliffe2002principal}. Once PCA is performed, we are left with an approximation of the original matrix that still contains valuable information, but with fewer dimensions. A single dimension is often a combination of variables from the initial matrix $M$, and should be independent from other dimensions. In WEKA, the PCA selects the minimum number of dimensions that covers at least the 95\% of the variance. 

\subsubsection{Classifier Selection}
\label{sec:Classifier}
CCP is independent of the specific classifier used in the model. In this first CPP version we therefore investigated the use of the following classifiers.

\noindent$\bullet$~{\bf Decision Tree}:
Decision Trees (DTs) are a supervised learning method used for classification and regression.  The goal is to create a model that predicts the type of a source file by learning simple decision conditions inferred from the words used in tactical files. In a decision tree, the internal nodes represent test conditions while leaf nodes represent categories.  In our case there are two categories of impacted and non-impacted classes. The attributes chosen to build the tree are based on information gain theory \cite{anyanwu2009comparative}, meaning that the internal nodes of the decision tree are constructed from the attributes that provide maximum information while the leaf node predicts a category or class. To increase the accuracy of the decision tree, most algorithms employ some form of pruning to remove branches of the tree that are less useful in performing classifications \cite{anyanwu2009comparative}.\vspace{4pt}\\
\noindent$\bullet$~{\bf Random Forest}:
The Random Forest classifier generates a number of separate, randomized decision trees are generated. It is similar to the bagging algorithm, but differs in that when creating decision trees, there is some randomness when choosing what feature to split on. In similar fashion to bagging, once all the trees have been generated, the nodes with the most consensus among the trees is chosen. This technique has proven to be highly accurate and robust against noise \cite{breiman2001random}. However, because this classifier requires the building of many different decision trees, it can be extremely expensive to run on large datasets.\vspace{4pt}\\
\noindent$\bullet$~{\bf N\"aive Bayes}:
The N\"aive Bayes classifier is a probabilistic classifier based on Bayes theorem and follows the assumption that the contribution of an individual feature towards deciding the probability of a particular class is independent of other features in that dataset instance \cite{mccallum1998comparison}. For example, in the case of detecting an impacted class, the contribution of the DIT metric is independent of the contribution of Requirements-to-Code similarity metric. Naive Bayes tends to overestimate the probability of the selected class.\vspace{4pt}\\
\noindent$\bullet$~{\bf Bayes Net}:
The Bayes Network classifier is based on a probabilistic graphical model that represents a set of random variables and their conditional dependencies via a Directed Acyclic Graph (DAG) with a set of Conditional Probability Tables (CPT) \cite{friedman1997bayesian}. The learning process of this classifier involves first learning the structure of DAG and then learning the probability tables. The classification is achieved by calculating the conditional probability for all class values given the observed value of metrics for each instance. \vspace{4pt}\\
\noindent$\bullet$~{\bf Logistic}:
The logistic classifier is built on a multinomial logistic regression model with a ridge estimator. Logistic regression model estimates the probabilities of the different possible outcomes of a categorically distributed dependent variable, given a set of independent variables. The estimation is performed through the logistic distribution function. The ridge estimator is used to improve the parameter estimation and to diminish future prediction error \cite{leCessie1992}.\vspace{4pt}\\
\noindent$\bullet$~{\bf Bagging}:
Bagging is an ensemble classifier. It trains individual classifiers on a random sampling of the original training set and then uses majority voting to attain the final results. Aggregation methods have been shown to be effective when used in conjunction with ``unstable'' learning algorithms such as decision trees where small changes in the training set result in large changes in predictions \cite{breiman1996bagging}.\vspace{4pt}\\

\subsubsection{Training the Classifier}
\label{sec:XValidation}
The generated profile was then used to train and test the CCP classifier using a cross-validation approach \cite{arlot2010survey}. In general, the adoption of cross-validation is a standard approach for assessing prediction models in order to obtain realistic and general results \cite{witten2005data, Kim:2011}. In a cross-validation approach, the data is split in N randomly separated chunks. In each iteration, N-1 chunks are used to train the classifier while one chunk is set aside for testing. During the testing step, the trained classifier is used to predict whether a class is impacted by a requirement or not.  The final accuracy results are computed after all N chunks had been tested.

==> DataExtractionOLD.tex <==
\section{Data Extraction}
\hilight{Currently a placeholder}
\subsection{Linking Process}
Unfortunately, most project management tools we tested are not directly linked to an SCM. Thus, the CCP linker must perform some data-processing to determine which data should be connected to which commits.

\begin{enumerate}
\item The linker attempts to link each requirement to one or more commits.
\item The linker calculates the approximate set of files present at the time of the requirement, as well as the number of files touched as a result of the requirement. 
\item Temporal locality is calculated (with care) for each requirement.
\item CCP then calculates the names and commit IDs of each release.
\item For each release, CCP performs static analysis.
\item For each requirement, its release ID is checked. CCP links release metrics to requirements that are part of that release.
\item Any externally computed metrics, such as VSM calculations, are linked in as well.
\end{enumerate}

The most central data structure in the linking process is that of a \emph{RequirementChange}. A RequirementChange is simply a textual requirement that can be directly linked to source code changes. Once the RequirementChange object construction has been completed, it will contain several linked commits, a list of files that were touched by those commits, and an approximate list of untouched files present in the system at the time of the requirement's creation. Each instance of a class being touched or untouched will be used as a sample in the finished dataset.

CCP relies on software developers following specific rules when performing commits: they must specify the full ID of the originating requirement when performing a commit. So, if a requirement is created named TIKA-11, the commit associated with the requirement must have TIKA-11 in its commit message. Assuming the project is named TIKA, the commit is evaluated with the regular expression:
\begin{lstlisting}.*TIKA-([0-9]+).*
\end{lstlisting}

This constraint is a reasonable and practical one and is assumed in numerous industrial bridges e.g. the Jira-GitHub link.  When CCP parses all of the commits, it will check each commit for a valid requirement ID. If a commit does not contain a valid requirement ID, it will not be linked. 

In order to determine the \emph{touched} files as a result of a requirement, we simply add up the number of changed files in the RequirementChange object's linked commits. We then determine the untouched files present at the time of the requirement by checking out the first commit to implement the requirement, looking at all its files, then filtering out any files that were created after the requirement date. We filter out any files that were present in our list of touched files. This is not a perfect procedure, but we found it less error-prone than other methods. 

Determining which commit is the first in a release can be difficult. Sometimes, users do not tag software releases properly in the SCM repository. Or, they create many extraneous ``tags'' that are not actually releases. We thus employ a heuristic in order to approximate the commit ID of a release. We assume that each requirement in the project management software is marked with a release ID. We then, using our set of linked requirements, look up the commit ID of the first requirement to implement that release and record its parent commit ID. If we did not take the parent commit of the first requirement in a release, we could risk effectively giving requirements data from the future, invalidating our data.

==> ImpactAnalysis.tex <==

\section{Impact Analysis}


Bohner modeled 

\subsection{Manual Impact Analysis}
From 1996 to the mid 2000’s, Shawn A. Bohner conducted a number of studies on impact analysis. In 1996, Bohner performed a study detailing ways to integrate impact analysis into the development process at the human level \cite{bohner1996software}.  In 2003, Bohner attempted a study of impact analysis in regards to changes to commercial off-the-shelp components . Keeping in mind the concepts of the starting impact set (the changes estimated to be made) and the actual impact set (the actual changes), Bohner detailed that software objects could be modeled as a dependency matrix or graph, from which one could look at both indirect and direct impacts. Each Software Lifecycle Object could be thought of as being a certain distance away from another SLO. SLOs that are a large distance from each other could be objects in different modules, so making a change to one unlikely to affect the other. SLOs that have a short distance are usually highly dependent on each other. With this measure of distance in mind, Bohner then observed that using 3D visualization techniques was useful in analyzing the actual impact sets. 



==> MOTIVATION.tex <==
\\ \\
*********** Start Motivation Discussion ***********************
\section{PLACEHOLDER DISCUSSION}
I'm a bit concerned that the current reasons/motivation aren't actually applicable to this paper.  They seem to be a perfect fit for the TSE one (which has the ability to look ahead), but they don't seem to apply to the work in this paper.  I think it would be a mistake to include these in the introduction (given that we can't deliver these benefits in the reduced part of the work we publish in this paper).  The current approach doesn't look ahead -- it just identifies the impact of the current requirement (we call it the "next" requirement) but the fact that we only look-ahead one requirement - really means it is the current requirement to be implemented.

Some specific comments:
\begin{itemize}
    \item Release Planning:  For this to be a motivation we need to be able to look ahead.  This paper doesn't do that.  Can we save the motivation for the TSE paper?
    \item Refactoring:  This also is dependent upon look-ahead -- if we suspect that a class is going to be touched many times in the future then we should refactor now.  But this paper doesn't attempt to look-ahead -- it just deals with the "next" requirement (which is in effect the current requirement).
    \item Effort and Defect estimation: Certainly impact analysis supports effort estimation.
\end{itemize}

So I wonder if we could refocus the benefits on what this paper delivers (instead of the broader benefits that we plan for our look-ahead in the future.We should brainstorm - but here are suggestions (extracted from Davide's earlier list).
\begin{itemize}
    \item More accurate identification of the right classes to modify.  Reduces the need for LATER (post-release modifications).  Enables a more strategic implementation of the change - with fewer unforeseen side effects.
    \item Strategic decision making (based on Effort estimation): If we have a more complete understanding of the impact of a change - we can better estimate effort and determine whether we should invest time making this change. 
\end{itemize}

******* END MOTIVATION DISCUSSION **************

==> OldTemporalLocality.tex <==
\subsection{Temporal Locality of Class Changes (TLCC)}
\label{sec:TLCC}
The third metric family, \emph{Temporal Locality of Class Changes} (TLCC), takes the modification history of a class into consideration. It is depicted in Figure \ref{fig:TempLocality}. Several authors have shown that change history is one of the strongest predictors of future change \cite{Graves:2000:PFI:347489.347496, DBLP:series/springer/ZimmermannNZ08} and that a class that has frequently changed in the past is more likely to change in the future. 
Previous research has shown that classes that have been frequently modified in the past are more likely to be impacted by future changes \cite{DBLP:series/springer/ZimmermannNZ08}. Furthermore, research has shown that more recent commits are stronger indicators of change than less recent ones.  Kim et al. pioneered the use of \emph{temporal locality} in predicting software change, building a variety of caches to weight the importance of prior software modifications \cite{kim2007predicting}. Bernstein et al. rolled up the number of modifications for a class by month for the most 6 recent months, and used those temporal metrics to train a defect-predicting classifier \cite{bernstein2007improving}. While TLCC works in a rather indirect way, we include it as one of our metric families because of its above-average performance in prior studies. Prior work has focused primarily on bug-fixing changes  while our emphasis in this paper is on source code changes resulting from the implementation of a new requirement.   

\begin{figure}[!t]  
    \begin{minipage}[b]{.95\linewidth}
     \centering
     \includegraphics[width=1.0\textwidth]{Metric3.pdf}
     \hspace{-20pt}
     \hspace{30pt}
   \end{minipage}  
    \caption{Temporal locality of requirements-associated changes made to the Class ({\bf TLCC})}
   \label{fig:TempLocality}
\end{figure} 

We compute TLCC in three different ways which represent three intuitive patterns of past source code change behavior.  In the following explanation, $k$ is the number of modifications applied to class $C$ and also the index of its oldest modification. $N$ is the total number of commits that were performed when $C$ existed. $i$ is the number of the current modification, where the least recent commit of $C$ has an index of 1. The closer the modification is to index 1, the more recent the modification, and the more weight it is given. The three metrics are defined as follows:\\

\begin{itemize}[-]
\itemsep-.1em
\item {\bf Simple Count Percent:} This divides the number of times class $C$ has been touched up until that point in the history by the total number of commits in which that class existed in the dataset. 
\begin{equation} 
TLCC_{SCP}(C) = {k}/{N} 
\end{equation}

\item {\bf Linear:}
This approach applies more weight to recent class modifications. Given that the most recent commit index is 1, the modification of the class at commit index 2 will be assigned a weight of 0.5, the modification at index 3 will be assigned the weight 1/3, etc. All of these weights are divided by the total number of commits from the creation of the class until the current point in time.
\begin{equation}
TLCC_{Lin}(C) = \frac {\sum_{i=1}^{k} \frac{1}{i}}{N} \
\end{equation}

\item {\bf Logarithmic:} Using a linear locality may assign insufficient weight to older modifications. In this approach we divide by $ln(k)$ when k is greater or equal to 3, allowing the weight to decrease more gradually. 
\begin{equation}
TLCC_{Log}(C) = \frac {\sum_{i=3}^{k} \frac{1}{ln(i)}}{N} \
\end{equation}
For example, a modification at commit index 4 will be given a weight of $1 / ln(4)$, the modification at commit index 5 will be given a weight of $1 / ln(5)$.  All weights are again divided by the total number of commits from the creation of the class until the current point in time.
\end{itemize}

\begin{table}[]
\centering
\setlength{\tabcolsep}{3pt}
\caption{Example of Temporal Locality Result for three classes. A commit that modifies the class is indicated as X, otherwise as 0.}
\label{tab:TemporalLocalityTable}
\begin{tabular}{|c||c|c|c|c|c|c||c|c|c|}
\hline
Class & \multicolumn{6}{c||}{Requirement Touch} & \multicolumn{3}{c|}{Temporal Locality Results} \\ \cline{2-10} 
Name & 1 & 2 & 3 & 4 & 5 & 6 & Simple & Linear & Logarithmic \\ \hline
A & X & X & X & X & 0 & 0 & \textbf{0.67} & 0.16 & \textbf{0.47} \\ \hline
B & 0 & 0 & X & X & X & 0 & 0.5 & 0.18 & 0.44 \\ \hline
C & 0 & 0 & 0 & 0 & X & X & 0.33 & \textbf{0.25} & 0.33 \\ \hline
\end{tabular}
\end{table}

To better understand the calculation and interpretation of temporal locality metrics, we provide a simple example. In Table \ref{tab:TemporalLocalityTable}, six different requirements have been implemented, possibly impacting three different classes. 
For the \emph{simple} calculation, class A has been touched four different times producing a score of $\approx$ 0.67 (i.e., 4/6). Class B has been touched three times for a score of 0.5, while Class C has a score of $\approx$ 0.33. 

\begin{table}[!t]
\setlength{\tabcolsep}{1pt}
\caption{Source Code Coupling, Cohesion, and Complexity metrics}
\label{tab:Codemetrics}
\begin{tabular}{|L{2.1cm}|L{1cm}|L{5cm}|}
\hline
\centering 
	Metric&Family&Description\\ \hline

	{\bf Com}\newline Complexity  &SQ&Counts number of key-words (e.g. if, else, for, while, etc. \cite{sonarsource2013sonarqube} (Complexity) \\ \hline
	{\bf NCLOC}\newline Size in lines of code&SQ&Counts number of lines of code (excluding white space and brackets). \cite{sonarsource2013sonarqube} (Size)\\ \hline
	{\bf Viol}\newline Violations &SQ& Number of rule violations (code smells). \cite{sonarsource2013sonarqube}. (Error Propensity)\\ \hline
	{\bf WMC}: Weighted Methods per Class&CKJM&Sums number of methods per class, weighted by the cyclomatic complexity for each method \cite{cho2001component}.  (Size, Complexity)\\ \hline
	{\bf DIT}: \newline Depth of Inheritance Tree &CKJM&Measures the number of levels in a class's inheritance tree. DIT is an indicator of code-reuse \cite{cho2001component}. (Coupling)\\ \hline
	{\bf NOC}: \newline Number of Children&CKJM&Measures the number of times a class has been subclassed \cite{cho2001component}.  (Coupling)\\ \hline
	{\bf CBO}: Coupling between Object Classes&CKJM&Measures the number of non-inheritance based associations to other classes \cite{cho2001component}.  (Coupling)\\ \hline
	{\bf RFC}: \newline Response for a Class&CKJM&Counts the methods that may be invoked by a class in response to an event \cite{cho2001component}.  (Coupling)\\ \hline
	{\bf LCOM}: \newline Lack of Cohesion of metrics&CKJM&Measures the extent to which methods in a class are internally cohesive \cite{cho2001component}.  (Cohesion)\\ \hline
	{\bf Ca}: \newline Afferent Couplings&CKJM&Measures the number of direct references from other classes \cite{cho2001component}. (Coupling)\\ \hline
	{\bf NPM}: Number of Public Methods&CKJM&Measures the number of publicly exposed methods \cite{cho2001component}. (Cohesion, Coupling)\\ \hline
	\end{tabular}
\end{table}

The linear method takes temporal locality of the class modification into consideration. Class A has been touched at its first, second, third, and fourth requirements. Class B has more recent modifications, but less total modifications than Class A; however, we can see that it still has a higher score at 0.18 than class A does.  Class C has the least total modification and the most recent modifications, but it has the highest linear temporal locality score at 0.25. This exemplifies how heavily the linear temporal locality method favors recent modifications.
The logarithmic method works very similarly to the linear one, but we can see that it penalizes older activity substantially less than the linear method. Specifically, the logarithmic metric suggests class A as the most prone to future change whereas the linear metric suggests class C. This is because in the linear method class A is highly penalized by the fact that it has not been touched by the last two requirements (5 and 6).
All three of these metrics are included in the TLCC metric family.

==> ParkingLot.tex <==
\begin{table}[!t]
\centering
\caption{Kruskal-Wallis pair-wise test results about the differences in a accuracy among the best configuration versus the other configurations. Significant results are in italic.}
\label{tab:PairwiseTest}
\begin{tabular}{|l|c|c|c|}
\hline
\multirow{2}{*}{Configuration} & \multicolumn{3}{c|}{Accuracy Metric}             \\ \cline{2-4} 
                               & Precision               & Recall                  & F1                      \\ \hline
None-Bagging                   & -                       & \textit{\textless.0001} & 0.234                   \\ \hline
None-BayesNet                  & \textit{\textless.0001} & -                       & \textit{\textless.0001} \\ \hline
None-J48                       & \textit{\textless.0001} & \textit{\textless.0001} & -                       \\ \hline
None-Logistic                  & \textit{\textless.0001} & \textit{\textless.0001} & \textit{\textless.0001} \\ \hline
None-NaiveBayes                & \textit{\textless.0001} & \textit{0.003}          & \textit{\textless.0001} \\ \hline
None-RandomForest              & \textit{0.0007}         & \textit{\textless.0001} & \textit{0.0034}         \\ \hline
PCA-Bagging                    & 0.0736                  & \textit{\textless.0001} & \textit{\textless.0001} \\ \hline
PCA-BayesNet                   & \textit{\textless.0001} & \textit{\textless.0001} & \textit{\textless.0001} \\ \hline
PCA-J48                        & \textit{\textless.0001} & \textit{\textless.0001} & \textit{\textless.0001} \\ \hline
PCA-Logistic                   & \textit{0.0018}         & \textit{\textless.0001} & \textit{\textless.0001} \\ \hline
PCA-NaiveBayes                 & \textit{\textless.0001} & \textit{\textless.0001} & \textit{\textless.0001} \\ \hline
PCA-RandomForest               & \textit{0.0001}         & \textit{\textless.0001} & \textit{\textless.0001} \\ \hline
\end{tabular}
\end{table}

%\subsection{Natural Language Processing}
%As the CCP system deals with textual requirement data, we utilized basic NLP techniques to synthesize our requirements data. Below is a summary of methods used in our textual pre-processing and similarity calculation steps.

%We followed a series of standard pre-processing steps to prepare the text \cite{jivani2011comparative}.  This involved removing non alpha-numeric characters, splitting CamelCase class, method, and variable names (e.g. camel case), and stemming each word to its morphological root using the Porter stemmer  \cite{jivani2011comparative}. 



We computed all of the metrics described in Chapther \ref{sec:Approach} of this paper at the point of the first commit for each release because it is impractical to run all metrics-gathering tools each time a new requirement is implemented. In effect, this means that the data available to our predictor is fresher in earlier phases of a release and becomes stale in later phases. We discuss this constraint in Section Y describing threats to validity.

A profile was then created for each project (\hilight{each release??}), in which a single row represented a pairwise combination of a requirement and a class (??). For each row, the profile captured each of the individual metric scores (e.g. various scores for class change history, scores representing the association between the requirement and the class, and the static analysis metrics). Finally, each row included a single cell documenting whether the class was actually touched when the requirement was introduced.

Unfortunately, most project management tools we tested are not directly linked to an SCM. Thus, the CCP linker must perform some data-processing to determine which data should be connected to which commits.

\begin{enumerate}
\item The linker attempts to link each requirement to one or more commits.
\item The linker calculates the approximate set of files present at the time of the requirement, as well as the number of files touched as a result of the requirement. 
\item Temporal locality is calculated (with care) for each requirement.
\item CCP then calculates the names and commit IDs of each release.
\item For each release, CCP performs static analysis.
\item For each requirement, its release ID is checked. CCP links release metrics to requirements that are part of that release.
\item Any externally computed metrics, such as VSM calculations, are linked in as well.
\end{enumerate}

The most central data structure in the linking process is that of a \emph{RequirementChange}. A RequirementChange is simply a textual requirement that can be directly linked to source code changes. Once the RequirementChange object construction has been completed, it will contain several linked commits, a list of files that were touched by those commits, and an approximate list of untouched files present in the system at the time of the requirement's creation. Each instance of a class being touched or untouched will be used as a sample in the finished dataset.


\end{lstlisting}

This constraint is a reasonable and practical one and is assumed in numerous industrial bridges e.g. the Jira-GitHub link.  When CCP parses all of the commits, it will check each commit for a valid requirement ID. If a commit does not contain a valid requirement ID, it will not be linked. 

In order to determine the \emph{touched} files as a result of a requirement, we simply add up the number of changed files in the RequirementChange object's linked commits. We then determine the untouched files present at the time of the requirement by checking out the first commit to implement the requirement, looking at all its files, then filtering out any files that were created after the requirement date. We filter out any files that were present in our list of touched files. This is not a perfect procedure, but we found it less error-prone than other methods. 

Determining which commit is the first in a release can be difficult. Sometimes, users do not tag software releases properly in the SCM repository. Or, they create many extraneous ``tags'' that are not actually releases. We thus employ a heuristic in order to approximate the commit ID of a release. We assume that each requirement in the project management software is marked with a release ID. We then, using our set of linked requirements, look up the commit ID of the first requirement to implement that release and record its parent commit ID. If we did not take the parent commit of the first requirement in a release, we could risk effectively giving requirements data from the future, invalidating our data.


%/// 
Our approach therefore determines the textual similarity between a new requirement and each of the existing requirements in the system.  It then uses these similarity scores to compute the similarity of the new requirement to the set of requirements associated with the change history of each class.  We constrained the set of associated requirements to 10, using only the ten most recent changes.

%\noindent $\bullet$~{\bf Rule Violations}
%The Sonarqube java plugin used in this project comes with over 1000 rules setup \cite{sonarsource2013sonarqube} including a number related to bad-smells such as \textit{private methods that do not access instance data should be static}, performance related, such as \textit{``wait(...)'' should be used instead of ``Thread. sleep(...)'' when a lock is held}, and security related, such as \textit{``public static'' fields should be constant}. We expect that if a class violates several of these rules, it is likely to need refactoring, and thus more likely to be changed. For each class file in a release, we measure the number of code quality rule violations.\vspace{12pt}\\
%\noindent$\bullet$~{\bf  Code Complexity}
%In addition we measured a variety of OO complexity metrics based on the intuitin that the more complex a class file is, the more likely it will need refactoring. The metrics reported in Table X were therefore computed for each individual release.



%as briefly 
%\hilight{Logic of refactoring doesn't fit this paper}
%Code complexity in Sonarqube is a simple measure of the number of key-words (if, else, for, while, etc.) used in a code fragment \cite{sonarsource2013sonarqube}.
        
%We expect that  \vspace{4pt}\\
%\noindent$\bullet$~{\bf Lines of Code}
%We expect that larger class files are more likely to be in need of refactoring. We measure the number of lines of code (excluding white space and curly braces) for each class file in each release.\vspace{4pt}\\
%\subsubsubsection{CKJM}
%\hilight{can someone introduce CKJM?}
%\noindent$\bullet$~{\bf CKJM WMC: Weighted methods per class}
%The WMC is the sum of the cyclocomatic complexities for each method in a class \cite{cho2001component}. If a class has 3 methods, with method foo having a complexity of 3, method bar having a complexity of 5, and method fizz having a complexity of 2, the WMC of the class will be 10. We expect that classes with complex methods are more likely to be refactored.\vspace{4pt}\\
%\noindent$\bullet$~{\bfDIT: Depth of Inheritance Tree}
%The DIT measures the number of levels in a class's inheritance tree. If one class extends another class in Java, the child class will possess the methods of the parent class. Thus, the DIT measure shows how much code re-use a class has \cite{cho2001component}. We expect that classes with higher DIT scores are less likely to be refactored. \vspace{4pt}\\
%\noindent$\bullet$~{\bf NOC: Number of Children}
%The NOC score measures the number of times a given class has been sub-classed. Sometimes in industry, a class can be implemented with poor abstraction, and its children need to make many custom member variables as a result, leading to more total sub-classes in the project \cite{cho2001component}. It is our hypothesis that classes with higher NOC scores are likely in need of refactoring, and thus more likely to be modified by the user.\vspace{4pt}\\
%\noindent$\bullet$~{\bf CBO: Coupling between object classes}
%For each class-file, CBO measures the number of non-inheritance related connections to other classes. Classes with a high CBO measure are generally much harder to modify, as modifications to the class in question can affect many other class files \cite{cho2001component}. We expect that classes with high CBO are likely in need of refactoring, and thus more likely to be modified. \vspace{4pt}\\
%\noindent$\bullet$~{\bf RFC: Response for a Class}
%The RFC is the count of all methods that can be invoked by a class in response to user input. A high RFC score is indicative of a class that will be difficult for developers to understand, and thus more time-consuming to modify. We expect that classes with high RFC scores are likely in need of refactoring, and thus more likely to be modified.\vspace{4pt}\\
%\noindent$\bullet$~{\bf LCOM: Lack of cohesion in methods}
%The LCOM score is used to measure the level of cohesion of methods in a class. If a class has many methods that operate on the same instance variables, it will have high cohesion. If a class has multiple methods that have no instance variables in common, it will have low cohesion \cite{cho2001component}. We expect that classes with low LCOM scores are likely in need of refactoring, and thus more likely to be modified.\vspace{4pt}\\
%\noindent$\bullet$~{\bf Ca: Afferent couplings}
 %For a given class, its afferent coupling score measures the amount of times that other classes in the project reference the given class. Classes with high afferent coupling scores are usually more difficult to modify, as sometimes many other coupled classes will need to be modified along with it \cite{cho2001component}.  We expect that classes with high afferent coupling scores are likely in need of refactoring, and thus more likely to be modified.\vspace{4pt}\\
%\noindent$\bullet$~{\bf NPM: Number of public methods}
%NPM in java measures the number of methods that have been exposed as public. Classes with many public methods can sometimes have poor cohesion, given that any accessing class can call the class's methods \cite{cho2001component}. We expect that classes with low LCOM scores are likely in need of refactoring, and thus more likely to be modified.







\section{Approach}
\label{sec:Approach}

\begin{figure}
\includegraphics[width=\columnwidth]{Overview.pdf}
\caption{An overview of the RCCP process (need to make consistent with Fig. 1.....)}
\label{fig:Overview}
\end{figure}

The goal of RCCP is to predict the set of classes that will be impacted by a new requirement. As depicted in Fig. \ref{fig:Overview}, RCCP extracts data from a source code repository (e.g. GitHub), and a requirements repository (e.g. Jira).  It then performs a series of processing steps to compute a set of metrics that are used to train the classifier. The metrics and logic for including them are described briefly:
\begin{itemize}
    \item {\bf Req2Reqs}: Metrics which computes the similarity between a new requirement and the set of requirements which have previously impacted a class. Much prior work has investigated the co-evolution of source code artifacts \cite{Girba:2007:UCA:1294948.1294970} \hilight{more refs}; however, here we explore co-evolution of requirements and code with the underlying assumption that a new requirement is likely to impact classes which have been previously impacted by one more more similar requirements.
    \item {\bf Req2Class}: Metrics which compute the similarity between a requirement and a specific class. Numerous publications have claimed that trace retrieval techniques which compute textual similarity between a requirement and a source code class serve as reliable predictor of change impact \cite{DBLP:conf/se/MaderE16, ICSMEMona}.
    \item {\bf Past History:} Metrics which determine the modification history of a class. Several authors have shown that change history is one of the strongest predictors of future change \cite{Graves:2000:PFI:347489.347496, DBLP:series/springer/ZimmermannNZ08} and that a class that has frequently changed in the past is more likely to change in the future. Howver, much prior work has focused on bug-fixing changes (\hilight{Hunt for NEW FEATURE CHANGES}); while our emphasis is on changes introduced by new features.
    \item {\bf SonarQube}: Metrics based upon code smells. Code smells are defined as symptoms in source code that are potentially indicative of a deeper problem \cite{DBLP:conf/icse/TufanoPBOPLP15}.  Code smells have a potentially strong correlation with bug fixes, because badly designed code may be more error prone, we include them in our suite of metrics based on the informal hypothesis that poorly designed areas of code may require a disproportionate amount of modifications during any source code change event.
    \item {\bf CKJM}: Metrics based upon Obect-Oriented coupling and cohesion. CKJM identifies a specific class of `bad smells' related to classes with particularly high coupling or low cohesion.  \hilight{add references and logic}.
\end{itemize}

 While the novel contribution of this paper is the new Req2Reqs family of metrics that take into consideration the historical impact of similar requirements, it would be n\"aive to focus on only a single type of metric. Throughout the remainder of this paper we therefore comparatively evaluate the efficacy of Req2Reqs as a stand-alone family of metrics as well as its efficacy within a suite of metrics composed from various combinations of the five metric groups.  
 Each group of metrics has several variants, all of which are described in depth in the follow section of the paper.  We evaluate the efficacy of each individual metric group, and each combination of metric groups, by training and evaluating a classifier to predict the set of impacted classes given a new requirement.  The training process involves several steps. First, raw requirements, classes, and commit logs are extracted from github and Jira.  From this data the metrics described in section \ref{sec:Metrics} are computed using a variety of different tools and techniques. The metrics are then used to train the classifier.  Once trained, the classifier can be used to support impact analysis of new requirement.  \hilight{Were we careful to only predict future impacts?}
 
 In this paper we address two \hilight{fix later} high-level research questions. As described later in the paper, each question is refined into a series of lower-level questions that support more indepth analysis of our approach.
 
 \begin{table*}[!t]
 \addtolength{\tabcolsep}{-4pt} 
\caption{Feature Requests serve as Requirements for the Accumulo System.  Requirements are associated with Classes during the Commit process.  The total set of requirements associated with a specific class over all commits in a given time period compose that class's Requirement Set}
\label{tab:Requirements}
\vspace{6pt}
\begin{tabular}{|L{1cm}|L{2.8cm}|L{7cm}|L{5.8cm}|}
\hline
{\bf Commit ID} & {\bf New Feature (aka Requirement)} & {\bf Requirement Description \newline (Only partial text shown here)}& {\bf Modified Classes \newline (per the GitHub commit log)}\\ \hline
2181 &  Organize tables on monitor page by namespace&Improve the look and feel of the monitor by using Twitter's bootstrap. & monitor/servlets/TablesServlet.java, monitor/util/Table.java \\ \hline
2998 & Provide a mechanism to allow clients to wait for balance &Wait for the balancer to run and find no work to do after creating a bunch of splits.& master/Master.java \\ \hline
1680 & Atomic add and remove of authorizations&Adding and removing an auth presents a race condition because of the two separate calls required to get, modify, then set the authorizations for a user...&shell/Shell.java, shell/commands/ DeleteAuthsCommand.java, shell/commands/DeleteAuthsCommandTest.java\\ \hline

\end{tabular}
\end{table*}

\begin{itemize}
    \item [\bf RQ1:] How effective is RCCP for predicting the impact of a new requirement upon source code classes?
    \item [\bf RQ2:] When used in combination with other types of metrics, does RCCP improve overall prediction accuracy?
\end{itemize} 

We investigate these research questions on four large open source Java projects.  Ultimately our results show that \emph{past history} of change is the biggest predictor of classes impacted by new functionality, while our new Req2Reqs metrics are the second strongest predictor.  Furthermore, we show that combining these two techniques leads to significant gains in accuracy.  \hilight{waiting on Davide's mega table} to finish discussion about results across four individual projects. 

%RCCP involves three primary steps:
%\setdefaultleftmargin{30pt}{}{}{}{}{}
%\begin{itemize}
%    \itemsep-.1em
%    \item [Step 1]{{\bf Code and requirements linkage}. Requirements are linked to commits and the first commit per %release is recorded.}% and serialize the results. During this step, we also extract the commit number of each %release.}
%    \item [Step 2]{{\bf Metrics measurement}. All metrics are computed for each commit, with the exception of temporal %locality which is measured once at the first commit of each revision level. This is due to the high computational resources required by the approach.}
%    \item [Step 3]{{\bf Metrics aggregation}. All metrics data is collated into a profile used to train the CCP classifier.}
%    \item [Step 4]{{\bf Prediction and evaluation}. Finally the CCP classifier is trained to predict the set of classes impacted by a new requirement. The predictor is evaluated for accuracy.}
%\end{itemize}
%Each of these steps are now described in greater detail.
%\setdefaultleftmargin{12pt}{0pt}{0pt}{0pt}{0pt}{0pt}

==> ResultsBACKUP.tex <==
\section{Results and Discussion}
\label{sec:Results}

We now discuss the findings with respect to each of the research questions. The first question (RQ1) asks ``How  effective  is  RCCP  for  predicting  the  impact  of  a  new  requirement  upon  source  code
classes?''  To answer this research question we compare the accuracy of predictions achieved using each of the five metrics groups individually for each of the four datasets.  Results are reported in Table \ref{tab:RQ1Results}.

\begin{table*}[]
\setlength{\tabcolsep}{2pt}
\centering
\caption{Accuracy of the five metric groups organized by classifier and dataset}
\label{tab:RQ1Results}
\begin{tabular}{|l|l|l|l|l|l|l|l|l|l|l|l|l|l|l|l|l|l|l|l|}
\hline
&&\multicolumn{3}{c|}{J48}&\multicolumn{3}{c|}{Random Forrest}&\multicolumn{3}{c|}{Bagging}&\multicolumn{3}{c|}{Naive Bayes}&\multicolumn{3}{c|}{Bayes Net}&\multicolumn{3}{c|}{Logistic Reg.}\\ \hline
&Metric&Rec&Pr&F1&Rec&Pr&F1&Rec&Pr&F1&Rec&Pr&F1&Rec&Pr&F1&Rec&Pr&F1\\ \hline
AC&ckjm&0&0&0&0&0&0.22&0&0&0&0&0&0&0&0&0&0&0&0\\ \hline
&Req2Code&0&0&0&0&0&0&0&0&0&0&0&0&0&0&0&0&0&0\\ \hline
&Req2Req&0&0&0&0&0&0.464&0&0&0&0&0&0&0&0&0&0&0&0\\ \hline
&SonarQB&0&0&0&0&0&0.14&0&0&0&0&0&0&0&0&0&0&0&0\\ \hline
&History&0&0&0&0&0&0.206&0&0&0&0&0&0&0&0&0&0&0&0\\ \hline
IG&ckjm&0&0&0&0&0&0.739&0&0&0&0&0&0&0&0&0&0&0&0\\ \hline
&Req2Code&0&0&0&0&0&0.729&0&0&0&0&0&0&0&0&0&0&0&0\\ \hline
&Req2Req&0&0&0&0&0&0.942&0&0&0&0&0&0&0&0&0&0&0&0\\ \hline
&SonarQB&0&0&0&0&0&0.741&0&0&0&0&0&0&0&0&0&0&0&0\\ \hline
&History&0&0&0&0&0&0.864&0&0&0&0&0&0&0&0&0&0&0&0\\ \hline
IS&ckjm&0&0&0&0&0&0&0&0&0&0&0&0&0&0&0&0&0&0\\ \hline
&Req2Code&0&0&0&0&0&0&0&0&0&0&0&0&0&0&0&0&0&0\\ \hline
&Req2Req&0&0&0&0&0&0.099&0&0&0&0&0&0&0&0&0&0&0&0\\ \hline
&SonarQB&0&0&0&0&0&0&0&0&0&0&0&0&0&0&0&0&0&0\\ \hline
&History&0&0&0&0&0&0.52&0&0&0&0&0&0&0&0&0&0&0&0\\ \hline
TK&ckjm&0&0&0&0&0&0.03&0&0&0&0&0&0&0&0&0&0&0&0\\ \hline
&Req2Code&0&0&0&0&0&0&0&0&0&0&0&0&0&0&0&0&0&0\\ \hline
&Req2Req&0&0&0&0&0&0&0&0&0&0&0&0&0&0&0&0&0&0\\ \hline
&SonarQB&0&0&0&0&0&0.015&0&0&0&0&0&0&0&0&0&0&0&0\\ \hline
&History&0&0&0&0&0&0.593&0&0&0&0&0&0&0&0&0&0&0&0\\ \hline
&History&0.555&0.555&0.555&0.555&0.555&0.555&0.555&0.555&0.555&0.555&0.555&0.555&0.555&0.555&0.555&0.555&0.555&0.555\\ 
\hline
\end{tabular}
\end{table*}

\hilight{NEED TO SEE THESE RESULTS FIRST}.
General observations: (placeholder)
\begin{itemize}
\item Trees do best.
\item History wins.
\item Req2Reqs comes second??
\end{itemize}

\hilight{Ton of text removed temporarily.} It is in the backup project.


Figure \ref{fig:RQ1Plots} reports the distributions of accuracy metrics of the six classifiers via box plots. Each box in Figure \ref{fig:RQ1Plots} represents 40 points, i.e., the 10 folds results for each of the four datasets. 
Table \ref{tab:RQ1} reports the accuracy of the six classifiers on the four datasets. Numbers in bold refers to the best classifier, i.e., the maximum value for a specific metric and dataset. According to Table \ref{tab:RQ1}, there is no single classifier that outperforms the others in all accuracy metrics and in all datasets. Only in the Ignite dataset there is a classifier (RandomForrest) that outperforms all the other classifiers in all metrics. In the remaining three datasets, the best classifier change across metrics. Moreover, the classifiers Bagging, J48 and RandomForest are better than BayesNet, Logistic and Naive Bayes, in all four datasets and three metrics. Finally, we note that J48 provides the highest F1 in all datasets other than Ignite.  

Regarding the accuracy of CCP over different datasets we can observe that Precision is much higher than Recall in all four datsets. This suggests that CCP is useful in scenarios such as suggesting classes to refactor, even though it may not identify all of the classes. Moreover, Ignite is clearly the dataset where CCP outperfrmed better in all accuracy metrics. This is probably due to the fact that Ignite is the only dataset that is almost balanced whereas  the other three datasets show a very low proportion of positives (see Table \ref{tab:Datasets}).

Table \ref{tab:AccuracyAgg} reports the aggregated accuracy of the six classifiers. We aggregated accuracies by weighting the datasets according to their size (See Table \ref{tab:Datasets}). According to Table \ref{tab:AccuracyAgg}, there is no single classifier that outperforms the others in all accuracy metrics. J48 provides the highest weighted F1 and therefore it is consdered the best overall classifier.

\begin{table}[]
\centering
\caption{Accuracy of CCP's different classifiers on different datasets.}
\label{tab:RQ1}
\begin{tabular}{|l|l|p{1.2cm}|p{1cm}|p{1cm}|}
\hline
Dataset                   & Classifier   & Mean Precision & Mean Recall & Mean F1 \\ \hline
\multirow{6}{*}{Accumulo} & Bagging      & \textbf{0.812}   & 0.442       & 0.572   \\ \cline{2-5} 
                          & BayesNet     & 0.243          & \textbf{0.630}       & 0.350   \\ \cline{2-5} 
                          & J48          & 0.760          & 0.470       & \textbf{0.580}   \\ \cline{2-5} 
                          & Logistic     & 0.528          & 0.015       & 0.028   \\ \cline{2-5} 
                          & NaiveBayes   & 0.108          & 0.574       & 0.182   \\ \cline{2-5} 
                          & RandomForest & 0.770          & 0.462       & 0.577   \\ \hline
\multirow{6}{*}{Ignite}   & Bagging      & 0.967          & 0.953       & 0.960   \\ \cline{2-5} 
                          & BayesNet     & 0.926          & 0.939       & 0.932   \\ \cline{2-5} 
                          & J48          & 0.962          & 0.951       & 0.957   \\ \cline{2-5} 
                          & Logistic     & 0.778          & 0.861       & 0.818   \\ \cline{2-5} 
                          & NaiveBayes   & 0.900          & 0.337       & 0.490   \\ \cline{2-5} 
                          & RandomForest & \textbf{0.971}   & \textbf{0.958}       & \textbf{0.964}   \\ \hline
\multirow{6}{*}{Isis}     & Bagging      & \textbf{0.885}   & 0.541       & 0.672   \\ \cline{2-5} 
                          & BayesNet     & 0.311          & \textbf{0.593}       & 0.408   \\ \cline{2-5} 
                          & J48          & 0.841          & 0.567       & \textbf{0.677}   \\ \cline{2-5} 
                          & Logistic     & 0.327          & 0.032       & 0.058   \\ \cline{2-5} 
                          & NaiveBayes   & 0.061          & 0.488       & 0.107   \\ \cline{2-5} 
                          & RandomForest & 0.846          & 0.472       & 0.606   \\ \hline
\multirow{6}{*}{Tika}     & Bagging      & 0.914          & 0.354       & 0.505   \\ \cline{2-5} 
                          & BayesNet     & 0.205          & 0.602       & 0.305   \\ \cline{2-5} 
                          & J48          & \textbf{0.922}          & 0.370       & \textbf{0.524}   \\ \cline{2-5} 
                          & Logistic     & 0.900          & 0.173       & 0.285   \\ \cline{2-5} 
                          & NaiveBayes   & 0.136          & \textbf{0.654}       & 0.225   \\ \cline{2-5} 
                          & RandomForest & 0.844          & 0.382       & 0.523   \\ \hline
\end{tabular}
\end{table}

% \begin{figure}
% \includegraphics[width=\columnwidth]{RQ1.pdf}
% \caption{Accuracy of CCP's different classifiers on different datasets.\hilight{Transform to a table from FaultPronePredictor3,TSE,DataAnalisi, New,RQ1,Stat.xlsx}}
% \label{fig:RQ1}
% \end{figure}

\begin{figure}
\includegraphics[width=\columnwidth]{H2F1.pdf}
\caption{F1 of different classifiers. Each distribuition relates to different folds and datasets (not weighted).}
\label{fig:RQ1Plots}
\end{figure}

\begin{table}[]
\centering
\caption{Weighted average accuracy of CCP's different classifier. The average is computed across results from four datasets weighted according to their size.}
\label{tab:AccuracyAgg}
\begin{tabular}{|l|p{1.95cm}|p{1.8cm}|p{1.2cm}|}
\hline
Classifier   & Weighted Mean Precision & Weighted Mean Recall & Weighted Mean F1 \\ \hline
Bagging      & \textbf{0.879}          & 0.537                & 0.665            \\ \hline
BayesNet     & 0.314                   & \textbf{0.604}       & 0.411            \\ \hline
J48          & 0.835                   & 0.562                & \textbf{0.671}   \\ \hline
Logistic     & 0.362                   & 0.047                & 0.071            \\ \hline
NaiveBayes   & 0.083                   & 0.496                & 0.123            \\ \hline
RandomForest & 0.840                   & 0.480                & 0.609            \\ \hline
\end{tabular}
\end{table}

% \begin{figure}
% \includegraphics[width=\columnwidth]{RQ1Agg.pdf}
% \caption{Weighted average accuracy of CCP's different classifier. The average is computed across results from four datasets weighted according to their size.\hilight{Transform to a table from FaultPronePredictor3,TSE,DataAnalisi, New,RQ1,Stat.xlsx}}
% \label{fig:AccuracyAgg}
% \end{figure}

Results from performing the Kruskal-Wallis test to evaluate null hypothesis H10 are reported in Table \ref{tab:RQ1H1} and show that we can reject H10 in 12 out of 12 cases. In other words, the accuracy of the classifiers in statistically different in the three accuracy metrics and in all four datasets.

\begin{table}[]
\centering
\caption{Kruskal-Wallis test results (p-values) about the differences in accuracy among classifiers over different datasets.}
\label{tab:RQ1H1}
\begin{tabular}{|l|l|l|l|}
\hline
Dataset  & Precision       & Recall          & F1              \\ \hline
Accumulo & \textless0.0001 & \textless0.0001 & \textless0.0001 \\ \hline
Ignite   & \textless0.0001 & \textless0.0001 & \textless0.0001 \\ \hline
Isis     & \textless0.0001 & \textless0.0001 & \textless0.0001 \\ \hline
Tika     & \textless0.0001 & \textless0.0001 & \textless0.0001 \\ \hline
\end{tabular}
\end{table}

% \begin{figure}
% \includegraphics[width=\columnwidth]{RQ1H1.pdf}
% \caption{Kruskal-Wallis test results (p-values) about the differences in accuracy among classifiers over different datasets.}
% \label{fig:RQ1H1}
% \end{figure}

Table \ref{tab:RQ1H2} reports the results from performing the Kruskal-Wallis test to comapare the best overal classifier (J48) with the other classifiers over different metrics and datasets. According to Table \ref{tab:RQ1H2} J48 is statistically better than BayesNet, Logistic, and Naive Bayes on all thre emetrics in all four datsets. Moreover, J48 is statistically better than Bagging in no datsets or metric. In conclusion we can reject H20 in 14 cases out of 20. 

\begin{table}[]
\centering
\caption{Kruskal-Wallis test results (p-values) about the differences in F1 between the best overall classifier (J48) and the other classifiers}
\label{tab:RQ1H2}
\begin{tabular}{|l|l|l|l|l|}
\hline
Classifier   & Accumulo & Ignite & Isis   & Tika   \\ \hline
Bagging      & 0.6232   & 0.0452 & 0.3075 & 0.6220 \\ \hline
BayesNet     & 0.0002   & 0.0002 & 0.0002 & 0.0002 \\ \hline
Logistic     & 0.0002   & 0.0002 & 0.0002 & 0.0004 \\ \hline
NaiveBayes   & 0.0002   & 0.0002 & 0.0002 & 0.0002 \\ \hline
RandomForest & 0.7913   & 0.0010 & 0.0002 & 0.7906 \\ \hline
\end{tabular}
\end{table}

% \begin{figure}
% \includegraphics[width=\columnwidth]{RQ1H2ByDataset.pdf}
% \caption{Kruskal-Wallis test results (p-values) about the differences in F1 between the best overall classifier (J48) and the other classifiers.}
% \label{fig:RQ1H2}
% \end{figure}









\subsection{RQ2: Does the use of historical associations improve the accuracy of CCP?}

Table \ref{tab:RQ2} reports the accuracy of the six classifiers on the four datasets when not using historical associations. Numbers in bold refers to the best classifier, i.e., the maximum value for a specific metric and dataset. According to Table \ref{tab:RQ2}, the classifiers Bagging, J48 and RandomForest are better than BayesNet, Logistic and Naive Bayes, in all four datasets and three metrics. 

Figure \ref{fig:RQ2Box} reports the box plots of the gain on Precision, Recall, and F1 provided by using historcal associations. Each box in Figure \ref{fig:RQ2Box} represents 40 points, i.e., the 10 folds results for each of the four datasets.  We computed Figure \ref{fig:RQ2Box} by subtracting from Figure \ref{fig:RQ1Plots} the accuracy of the classifiers when not using historical associations. According to Figure \ref{fig:RQ2Box} the gain provided by using histical associations is both positive and negative in all classifiers in all three metrics. In order to better understand the gain we analyze it for each dataset.

\begin{figure}
\includegraphics[width=\columnwidth]{RQ2F1.pdf}

\caption{F1 provided by classifiers using historical associations. Each distribuition relates to different folds and datasets (not weighted)}
\label{fig:RQ2Box}
\end{figure}


Table \ref{tab:RQ2Diff} reports the gain provided by using the historical associations in different classifiers over different datasets. We computed Figure \ref{tab:RQ2Diff} by subtracting Table \ref{tab:RQ2} to \ref{tab:RQ1}. Positive numbers refers to cases where the historical associations improved accuracy, for a given metric (column) on a given combination of classifier and dataset (row). Because we count 58 positive number we conclude that the use of historical associations improved the accuracy of the CCP in 58 out of 72 cases. Numbers in bold in Table \ref{tab:RQ2Diff} refers to the best classifier, i.e., the maximum value for a specific metric and dataset, when historical associations are not used. As we can see, all numbers in bold related to the F1 column are positive. This means that, in all four datasets, the use of the historical associations improved the accuracy of the best overal classifier. Moreover, the gain is positive also in Bagging and RandomForest which are, togheter with J48, much more accurate than the other classifiers. Therefore we can conclude that the use of historical associations  improve the accuracy of accurate clasifiers (i.e., the classiefiers that are usable).


\begin{table}[]
\centering
\caption{Average accuracy of the CCP when not using the historical associations over different classifiers and datasets}
\label{tab:RQ2}
\begin{tabular}{|l|l|p{1.2cm}|p{1cm}|p{1cm}|}
\hline
Dataset                   & Classifier   & Mean Precision & Mean Recall    & Mean F1        \\ \hline
\multirow{6}{*}{Accumulo} & Bagging      & \textbf{0.768} & 0.245          & 0.371          \\ \cline{2-5} 
                          & BayesNet     & 0.304          & \textbf{0.265} & 0.282          \\ \cline{2-5} 
                          & J48          & 0.753          & 0.248          & \textbf{0.372} \\ \cline{2-5} 
                          & Logistic     & 0.327          & 0.003          & 0.006          \\ \cline{2-5} 
                          & NaiveBayes   & 0.099          & 0.208          & 0.134          \\ \cline{2-5} 
                          & RandomForest & 0.422          & 0.243          & 0.308          \\ \hline
\multirow{6}{*}{Ignite}   & Bagging      & 0.828          & 0.861          & 0.844          \\ \cline{2-5} 
                          & BayesNet     & 0.767          & 0.720          & 0.743          \\ \cline{2-5} 
                          & J48          & \textbf{0.834} & 0.858          & \textbf{0.845} \\ \cline{2-5} 
                          & Logistic     & 0.614          & \textbf{0.867} & 0.719          \\ \cline{2-5} 
                          & NaiveBayes   & 0.796          & 0.242          & 0.371          \\ \cline{2-5} 
                          & RandomForest & 0.784          & 0.811          & 0.797          \\ \hline
\multirow{6}{*}{Isis}     & Bagging      & \textbf{0.875} & 0.506          & 0.641          \\ \cline{2-5} 
                          & BayesNet     & 0.429          & 0.441          & 0.435          \\ \cline{2-5} 
                          & J48          & 0.838          & \textbf{0.531} & \textbf{0.650} \\ \cline{2-5} 
                          & Logistic     & 0.354          & 0.036          & 0.065          \\ \cline{2-5} 
                          & NaiveBayes   & 0.115          & 0.273          & 0.161          \\ \cline{2-5} 
                          & RandomForest & 0.828          & 0.460          & 0.591          \\ \hline
\multirow{6}{*}{Tika}     & Bagging      & 0.944          & 0.305          & 0.452          \\ \cline{2-5} 
                          & BayesNet     & \textbf{0.955} & 0.169          & 0.283          \\ \cline{2-5} 
                          & J48          & 0.819          & \textbf{0.357} & \textbf{0.492} \\ \cline{2-5} 
                          & Logistic     & \textbf{0.955} & 0.169          & 0.283          \\ \cline{2-5} 
                          & NaiveBayes   & 0.166          & 0.064          & 0.087          \\ \cline{2-5} 
                          & RandomForest & 0.866          & 0.277          & 0.413          \\ \hline
\end{tabular}
\end{table}

% \begin{figure}
% \includegraphics[width=\columnwidth]{RQ2.pdf}
% \caption{Average accuracy of the CCP when not using the historical associations over different classifiers and datasets}
% \label{fig:RQ2}
% \end{figure}

\begin{table}[]
\centering
\caption{Gain provided by the use of historical associations of different classifiers on different datasets.}
\label{tab:RQ2Diff}
\begin{tabular}{|l|l|p{1.2cm}|p{1cm}|p{1cm}|}
\hline
Dataset                   & Classifier   & Mean Precision  & Mean Recall     & Mean F1        \\ \hline
\multirow{6}{*}{Accumulo} & Bagging      & \textbf{0.044}  & 0.197           & \textbf{0.201} \\ \cline{2-5} 
                          & BayesNet     & -0.061          & \textbf{0.365}  & 0.068          \\ \cline{2-5} 
                          & J48          & 0.007           & 0.222           & 0.208          \\ \cline{2-5} 
                          & Logistic     & 0.201           & 0.012           & 0.023          \\ \cline{2-5} 
                          & NaiveBayes   & 0.009           & 0.367           & 0.047          \\ \cline{2-5} 
                          & RandomForest & 0.348           & 0.219           & 0.269          \\ \hline
\multirow{6}{*}{Ignite}   & Bagging      & 0.139           & 0.092           & 0.116          \\ \cline{2-5} 
                          & BayesNet     & 0.159           & 0.218           & 0.189          \\ \cline{2-5} 
                          & J48          & \textbf{0.128}  & 0.094           & \textbf{0.111} \\ \cline{2-5} 
                          & Logistic     & 0.164           & \textbf{-0.006} & 0.099          \\ \cline{2-5} 
                          & NaiveBayes   & 0.104           & 0.095           & 0.119          \\ \cline{2-5} 
                          & RandomForest & 0.187           & 0.147           & 0.167          \\ \hline
\multirow{6}{*}{Isis}     & Bagging      & \textbf{0.010}  & 0.036           & 0.031          \\ \cline{2-5} 
                          & BayesNet     & -0.118          & 0.152           & -0.027         \\ \cline{2-5} 
                          & J48          & 0.003           & \textbf{0.035}  & \textbf{0.027} \\ \cline{2-5} 
                          & Logistic     & -0.027          & -0.004          & -0.007         \\ \cline{2-5} 
                          & NaiveBayes   & -0.054          & 0.215           & -0.054         \\ \cline{2-5} 
                          & RandomForest & 0.017           & 0.012           & 0.015          \\ \hline
\multirow{6}{*}{Tika}     & Bagging      & -0.029          & 0.048           & 0.053          \\ \cline{2-5} 
                          & BayesNet     & \textbf{-0.750} & 0.434           & 0.022          \\ \cline{2-5} 
                          & J48          & 0.102           & \textbf{0.012}  & \textbf{0.032} \\ \cline{2-5} 
                          & Logistic     & \textbf{-0.055} & 0.004           & 0.002          \\ \cline{2-5} 
                          & NaiveBayes   & -0.030          & 0.590           & 0.138          \\ \cline{2-5} 
                          & RandomForest & -0.023          & 0.105           & 0.111          \\ \hline
\end{tabular}
\end{table}

% \begin{figure}
% \includegraphics[width=\columnwidth]{RQ2Diff.pdf}
% \caption{Gain provided by the use of historical associations of different classifiers on different datasets.}
% \label{fig:RQ2Diff}
% \end{figure}

Table \ref{tab:RQ2Weig} reports the aggregated accuracy of the six classifiers when not using historical associations. We aggregated accuracies by weighting the datasets according to their size (See Table \ref{tab:Datasets}). According to Figure \ref{tab:RQ2Weig}, the best CCP classifier, when not using historical associations, is J48, which coincides with the best CCP classifier when using all the data. Note that, according to Table \ref{tab:RQ2} J48 resulted as the best overal classifier in three out of four datasets.

Table \ref{tab:RQ2WeigDiff} reports the gain on weighted average accuracy of the six classifiers. We computed Table \ref{tab:RQ2WeigDiff} by subtracting Table \ref{tab:RQ2Weig} to \ref{tab:AccuracyAgg}. Positive numbers refers to cases where the historical associations improve weighted average  accuracy on a classifier. Numbers in bold refer to the best classifiers. Because all bold numbers are postivies we conclude that the use of historical associations improved the weighted average accuracy for the best classifiers. 

\begin{table}[]
\centering
\caption{Weighted average accuracy of different classifiers when not using the historical associations.}
\label{tab:RQ2Weig}
\begin{tabular}{|l|p{1.95cm}|p{1.8cm}|p{1.2cm}|}
\hline
Classifier   & Weighted Mean Precision & Weighted Mean Recall & Weighted Mean F1 \\ \hline
Bagging      & \textbf{0.862}          & 0.482                & 0.613            \\ \hline
BayesNet     & 0.425                   & 0.425                & 0.423            \\ \hline
J48          & 0.828                   & \textbf{0.505}       & \textbf{0.622}   \\ \hline
Logistic     & 0.360                   & 0.049                & 0.072            \\ \hline
NaiveBayes   & 0.126                   & 0.263                & 0.162            \\ \hline
RandomForest & 0.782                   & 0.441                & 0.562            \\ \hline
\end{tabular}
\end{table}

% \begin{figure}
% \includegraphics[width=\columnwidth]{RQ2Weig.pdf}
% \caption{Weighted average accuracy of different classifiers when not using the historical associations.}
% \label{fig:RQ2Weig}
% \end{figure}

\begin{table}[]
\centering
\caption{Gain on weighted average accuracy provided by using histirical associations on different classifiers.}
\label{tab:RQ2WeigDiff}
\begin{tabular}{|l|p{1.95cm}|p{1.8cm}|p{1.2cm}|}
\hline
Classifier   & Weighted Mean Precision & Weighted Mean Recall & Weighted Mean F1 \\ \hline
Bagging      & \textbf{0.016}          & 0.054                & 0.052            \\ \hline
BayesNet     & -0.110                  & \textbf{0.179}       & -0.012           \\ \hline
J48          & 0.006                   & 0.057                & \textbf{0.049}   \\ \hline
Logistic     & 0.002                   & -0.002               & -0.002           \\ \hline
NaiveBayes   & -0.043                  & 0.232                & -0.038           \\ \hline
RandomForest & 0.058                   & 0.038                & 0.047            \\ \hline
\end{tabular}
\end{table}

% \begin{figure}
% \includegraphics[width=\columnwidth]{RQ2WeigDiff.pdf}
% \caption{Gain on weighted average accuracy provided by using histirical associations on different classifiers.}
% \label{fig:RQ2WeigDiff}
% \end{figure}

Table \ref{tab:RQ2H3} reports the statistical test results about the differences in accuracy of the best overall classifier (J48), over different datasets, when using versus not using the historical associations. According to Table \ref{tab:RQ2H3}, the use of historical associations statistically improves the accuracy of the best overal classifier  in Recall and F1 in all four datasets and in Precision in two out of four metrics. Therefore, we can reject H30 in 10 out of 12 cases.

\begin{table}[]
\centering
\caption{Kruskal-Wallis test results about the differences in accuracy of the best overall classifier (J48), over different datasets, when using versus not using the historical associations}
\label{tab:RQ2H3}
\begin{tabular}{|l|r|r|r|}
\hline
Dataset  & Precision       & Recall          & F1              \\ \hline
Accumulo & 0.0399          & \textless0.0001 & \textless0.0001 \\ \hline
Ignite   & \textless0.0001 & \textless0.0001 & \textless0.0001 \\ \hline
Isis     & 0.4243          & \textless0.0001 & \textless0.0001 \\ \hline
Tika     & \textless0.0001 & \textless0.0001 & \textless0.0001 \\ \hline
\end{tabular}
\end{table}

% \begin{figure}
% \includegraphics[width=\columnwidth]{RQ2H3.pdf}
% \caption{Kruskal-Wallis test results about the differences in accuracy of the best overall classifier (J48), over different datasets, when using versus not using the historical associations}
% \label{fig:RQ2H3}
% \end{figure}


\subsection{RQ3: How does  the accuracy of CCP vary according to groups of metrics?}

\subsubsection{Which is the most accuarate single group of metrics?}


Table \ref{tab:RQ3only1Group} reports the F1 achieved by the best classifier for each single group of metrics for different datasets. According to Table \ref{tab:RQ3only1Group} the most accurate group of metric is Historical Association (i.e., ReqSim) in Accumulo and Ignite and it is Temporal Locality in Isis and Tika. We note that RandomForrest is the most accurate classifier in the best sinhgle group of metrics in all four dataset whereas J48 is the most accurate clasifier in no group of metric or dataset. This sugegsts the use of RandomForest over J48 when using a small number of metrics.

Table \ref{tab:RQ3Weig} reports the F1 weighted average F1 achieved  each single group of metrics when used to its best classifier. According to Table \ref{tab:RQ3Weig} the most accurate group of metric is Temporal Locality and the second best is Historical Associations. We note that Historical Associations resulted prety low in Isis which, being the biggest dataset, higly decrea3ed the weighted average.

% Please add the following required packages to your document preamble:
% \usepackage{multirow}
\begin{table}[]
\centering
\caption{Accuracy provided by the best classifier for each single group of metrics for different datasets}
\label{tab:RQ3only1Group}
\begin{tabular}{|l|l|l|p{1.2cm}|}
\hline
Dataset                   & GroupName        & Classifier   & Max Mean-F1     \\ \hline
\multirow{5}{*}{Accumulo} & ckjm             & RandomForest & 0.2203          \\ \cline{2-4} 
                          & codeSim          & NaiveBayes   & 0.1180          \\ \cline{2-4} 
                          & reqSim           & RandomForest & \textbf{0.4642} \\ \cline{2-4} 
                          & sonarqube        & RandomForest & 0.1395          \\ \cline{2-4} 
                          & temporalLocality & RandomForest & 0.2057          \\ \hline
\multirow{5}{*}{Ignite}   & ckjm             & Logistic     & 0.7388          \\ \cline{2-4} 
                          & codeSim          & Logistic     & 0.7287          \\ \cline{2-4} 
                          & reqSim           & RandomForest & \textbf{0.9423} \\ \cline{2-4} 
                          & sonarqube        & Logistic     & 0.7407          \\ \cline{2-4} 
                          & temporalLocality & RandomForest & 0.8640          \\ \hline
\multirow{5}{*}{Isis}     & ckjm             & NaiveBayes   & 0.0500          \\ \cline{2-4} 
                          & codeSim          & NaiveBayes   & 0.0425          \\ \cline{2-4} 
                          & reqSim           & RandomForest & 0.0992          \\ \cline{2-4} 
                          & sonarqube        & NaiveBayes   & 0.0354          \\ \cline{2-4} 
                          & temporalLocality & RandomForest & \textbf{0.5199} \\ \hline
\multirow{5}{*}{Tika}     & ckjm             & RandomForest & 0.0302          \\ \cline{2-4} 
                          & codeSim          & NaiveBayes   & 0.0734          \\ \cline{2-4} 
                          & reqSim           & BayesNet     & 0.2961          \\ \cline{2-4} 
                          & sonarqube        & RandomForest & 0.0154          \\ \cline{2-4} 
                          & temporalLocality & RandomForest & \textbf{0.5937} \\ \hline
\end{tabular}
\end{table}

% \begin{figure}
% \includegraphics[width=\columnwidth]{RQ3.pdf}
% \caption{Accuracy provided by the best classifier for each single group of metrics for different datasets. }
% \label{fig:RQ3only1Group}
% \end{figure}


\begin{table}[]
\centering
\caption{Average weighted accuracy provided by the different single groups of metrics using their best classfiers.}
\label{tab:RQ3Weig}
\begin{tabular}{|p{1.75cm}|p{0.6cm}|p{0.88cm}|p{0.72cm}|p{0.7cm}|p{1.2cm}|}
\hline
              & ckjm   & codeSim & reqSim & sonar- qube & temporal- Locality \\ \hline
Weighted Max Mean-F1 & 0.0821 & 0.0643  & 0.1574 & 0.0604    & 0.4919           \\ \hline
\end{tabular}
\end{table}

% \begin{figure}
% \includegraphics[width=\columnwidth]{RQ3Weig.pdf}
% \caption{Average weighted accuracy provided by the different single groups of metrics using their best classfiers. }
% \label{fig:RQ3Weig}
% \end{figure}


\subsubsection{Which are the best combinations of groups of metrics?}

Table \ref{tab:RQ32Table} reports the best combinations of groups of metrics, and their  weighted average accuracy, when the number of groups varies from one to five. 
Table \ref{tab:RQ32Table}, the group Historical Associatinos is used in all four best combinations and therefore it is the most supportive group after temporal locality. 

\begin{table}[]
\centering
\caption{Best combinations of groups of metrics, related best classifier and weighted average accuracy of CCP, with the number of groups of metric varying from one to five. \hilight{this table will probably be replaced by a full table}}
\label{tab:RQ32Table}
\begin{tabular}{|p{3.5cm}|l|p{1.5cm}|}
\hline
Metrics                          & Best Classifier & Weighted Mean-F1 \\ \hline
temporalLocality                                   & RandomForest & 0.4919 \\ \hline
reqSim, temporalLocality                           & RandomForest & 0.6065 \\ \hline
reqSim, temporalLocality, ckjm                     & Bagging      & 0.6450 \\ \hline
codeSim, reqSim, temporalLocality, ckjm            & J48          & 0.6643 \\ \hline
codeSim, reqSim, temporalLocality, sonarqube, ckjm & J48          & 0.6707 \\ \hline
\end{tabular}
\end{table}

% \begin{figure}
% \includegraphics[width=\columnwidth]{RQ32Table.pdf}
% \caption{ Best combinations of groups of metrics, related best classifier and weighted average accuracy of CCP, with the number of groups of metric varying from one to five. \hilight{this table will probably be replaced by a full table}}
% \label{fig:RQ32Table}
% \end{figure}

\subsubsection{Are all groups of metrics important?}

Figure \ref{fig:RQ32PictureDatasets} reports the weighted  average F1 achieved by the best classifier using the best combination of groups of metrics, with the number of groups of metrics varying from one to five. According to Figure \ref{fig:RQ32PictureDatasets}, when the number of groups increases,...


Table \ref{tab:RQ3Stat2} reports the test results about the differences in accuracy among CCP when the number of groups of metrics increases incrementally from 1 to 5. According to Table \ref{tab:RQ3Stat2} ...

\begin{figure}
\includegraphics[width=\columnwidth]{RQ32PictureDatasets.pdf}
\caption{Weighted average F1 achieved by the best classifier using the best combination of groups of metrics, with the number of groups of metrics varying from one to five.}
\label{fig:RQ32PictureDatasets}
\end{figure}

\begin{table*}[t]
  \centering
\caption{Kruskal-Wallis test results about the differences in accuracy among CCP when when the number of groups of metrics increases incrementally from 1 to 5. Significant results are in italics. \hilight{add a table like this for each dataset}}
\label{tab:RQ3Stat2}
\begin{tabular}{|l|l|l|l|l|l|l|l|l|l|l|l|l|}
\hline
\multicolumn{1}{|c|}{\multirow{2}{*}{Dataset}} & \multicolumn{3}{c|}{1 vs. 2} & \multicolumn{3}{c|}{2 vs. 3} & \multicolumn{3}{c|}{3 vs. 4} & \multicolumn{3}{c|}{4 vs. 5} \\ \cline{2-13} 
\multicolumn{1}{|c|}{}                         & Precision  & Recall & F1     & Precision  & Recall & F1     & Precision  & Recall & F1     & Precision  & Recall & F1     \\ \hline
Accumulo                                       & 0.0003     & 0.0003 & 0.0003 & 0.0002     & 0.0002 & 0.0002 & 0.0091     & 0.1505 & 0.8501 & 0.4604     & 0.0685 & 0.1004 \\ \hline
Ignite                                         & 0.0002     & 0.2896 & 0.0002 & 0.0539     & 0.0008 & 0.0028 & 0.0257     & 0.7621 & 0.0312 & 0.2819     & 0.3307 & 0.8070  \\ \hline
Isis                                           & 0.0002     & 0.0002 & 0.0002 & 0.0002     & 0.0002 & 0.0002 & 0.0036     & 0.0010  & 0.0036 & 0.5745     & 0.2197 & 0.1815 \\ \hline
Tika                                           & 0.1838     & 0.0002 & 0.0002 & 0.1794     & 0.0857 & 0.0367 & 0.0209     & 0.0717 & 0.3252 & 0.2176     & 0.9791 & 0.7629 \\ \hline
\end{tabular}
\end{table*}


% \begin{figure}
% \includegraphics[width=\columnwidth]{RQ3Stat2.pdf}
% \caption{Kruskal-Wallis test results about the differences in accuracy among CCP when when the number of groups of metrics increases incrementally from 1 to 5. Significant results are in italics. \hilight{add a table like this for each dataset}}
% \label{fig:RQ3Stat2}
% \end{figure}

==> ResultsOld.tex <==
\begin{figure*}[!t]
   \begin{minipage}[b]{.45\linewidth}
     \centering
     \includegraphics[width=1.0\textwidth]{Rq1Accumulo.pdf}
     \hspace{-20pt}
     \subcaption{Accumulo}\label{fig:RQ1Accumulo}
     \hspace{30pt}
   \end{minipage}
  \begin{minipage}[b]{.45\linewidth}
     \centering
     \includegraphics[width=1.0\textwidth]{Rq1Ignite.pdf}
     \hspace{-20pt}
     \subcaption{Ignite}\label{fig:RQ1Ignite}
     \hspace{30pt}
   \end{minipage}
   
    \begin{minipage}[b]{.45\linewidth}
     \centering
     \includegraphics[width=1.0\textwidth]{Rq1Isis.pdf}
     \hspace{-20pt}
     \subcaption{Isis}\label{lab:RQ1Isis}
     \hspace{30pt}
   \end{minipage}     
   \begin{minipage}[b]{.45\linewidth}
     \centering
     \includegraphics[width=1.0\textwidth]{Rq1Tika.pdf}
     \hspace{-20pt}
     \subcaption{Tika}\label{lab:RQ1Tika}
     \hspace{30pt}
   \end{minipage}  
   
   \caption{F2-Metric achieved using five different classifiers from all combinations of features families in each data-set. Please note that the {\bf y-axis scale} varies among sub-figures.}
   \label{fig:AllMetrics}
\end{figure*}

\section{Results and Discussion}
\label{sec:Results}
We now discuss the findings with respect to each of the research questions. 

\subsection{RQ1: Which is the most accurate classifier?}
\hilight{This is now pretty large. The most informative information are in Figures 5 and 6 and therefore, if you want to reduce this RQ I suggest to remove Fig 3 and/or 4.}

Figure \ref{fig:rq1} reports the F2 achieved by each of the five different classifiers in all combinations of features in all four data-sets. According to Figure \ref{fig:rq1}:\\
-There is a high overlap among the different classifiers. Therefore, it is interesting to invesitigate if there is a best classifier for each different dataset. \\
-Random forrest resulted the classifier in average more accurate than the others. Therefore, it is interesting to investigate the extent of the difference in accuricay between RandomForest and the best classifier for the specific combination of families of features and dataset.\\

Figure \ref{fig:AllMetrics} reports the F2  achieved using five different classifiers from all combinations of features families in each data-set. According to Figure \ref{fig:AllMetrics}:\\
-The best classifier in average among combinations of feature families is RandomForrest for Accumulo and Tika, Logistic for Ignite and Bagging for Isis.


Figure \ref{fig:RQ1H1and2b} reports hypotheses testing on the difference between the accuracy of classifiers as measured with F2 on the same dataset.  An "x" denotes a pvalue lower than alpha (i.e., > 0.0125), and hence a rejection of an hypothesis. An "-" denotes the best classifier for a dataset. According to \ref{fig:RQ1H1and2b}:\\
-There is a significant difference in the accuracy provided by the differnet classifiers in all four datasets (see column 2). Therefore, we can reject H10 in all four cases.\\
-The accuray of the classifiers in Ignite is different than in other datsets. Specifically, in Ignite Logistic is significnatly better than all other classifiers whereas Logistic resulted significantly worse in the other three datasets.\\
-Except for Ignite, both RandomForrest and Bagging results or the best or not sifgnificanly different from the best and hence they seem to be a reliable choice.\\
-We can reject H20 in 10 out of 20 cases. Thus we can conclude that the best classifier is better than the others for almost half of the classifiers and datasets.\\



\begin{figure}
\includegraphics[width=\columnwidth]{RQ1H1and2b.pdf}
\caption{Hypotheses testing on the difference between the accuracy of classifiers as measured with F2 on the same dataset. An "x" denotes a pvalue lower than alpha (i.e., > 0.01), and hence a rejection of an hypothesis. An "-" denotes the best classifier, this is used for comparison in H20.}
\label{fig:RQ1H1and2b}
\end{figure}

Figure \ref{fig:RelativeF2withRF} reports the relative F2 achieved by the best overall classifier (RandomForest) in respect to the F2 achieved by the best classifier for a specific family group in a speicific data-set. The relative F2 has been computed as F2 of RandomForest divided by the F2 of the best classifier. The best classifier has been chosen as the one with the highest F2 for each specific combination of family features in each  specific dataset. According to \ref{fig:RelativeF2withRF}:\\ 
-RandomForest get in average among datasets and combinations of features families 93\% of the F2 compared to the best classifier.\\
-In Tika and Accumulo RandomForest gets at least 90%.\\
-There are combinatins of features families in Ignite and Isis where Randomforest gets only 70\% of the F2.\\
Because 70\% is not acceptable, we need to use the best classifier for the specific combination of features family when investigating Rq2 and RQ3. \\



\begin{figure}
\includegraphics[width=\columnwidth]{RelativeF2withRF.pdf}
\caption{Relative F2 achieved by the best overall classifier (RandomForest) in respect to the F2 achieved by the best classifier for a specific family group in a speicific data-set.}
\label{fig:RelativeF2withRF}
\end{figure}


\subsection{RQ2: which is the best single group of features?}
The second question (RQ2) asks ``How  effective  is  RCCP  for  predicting  the  impact  of  a  new  requirement  upon  source  code
classes?''  To answer this research question we compare the accuracy of predictions achieved using each of the five features groups individually for each of the four datasets. Because each features group can be used in combnation of different classifiers, and because according to RQ1 we do not have a dominant classifers, then we report the maximum accuracy of each single group of metrics among the five classifiers. The name of the classifiers resulting with the highest F2 are reported in the appendix (Ref..).

Results According to  Figure \ref{fig:RQ2f2}:
-Req2Req resulted the most accurate in two out of four datasets.
-TemporalLocality resulted the most accurate in the other two datasets.
-Req2Req resulted the most accurate in the datsets where the accuracy is resonably high.
-Req2Req resulted better than dummy in all four datasets. 
-CKJM and TemporalLocality resulted better than dummy in all datasets except for the easy one.
-In general the performances of the approach using one group of features only is not much better than a complete random approach. This results ask for checking the different combinations of groups of features.

\begin{figure}
\includegraphics[width=\columnwidth]{RQ2f2.pdf}
\caption{F2 (maximum among classifiers) of single groups of features on different datasets.}
\label{fig:RQ2f2}
\end{figure}

\begin{figure}
\includegraphics[width=\columnwidth]{RQ2RF.pdf}
\caption{F2 of RandomForest of single groups of features on different datasets.}
\label{fig:RQ2f2}
\end{figure}




Results According to Figure \ref{fig:RQ2GainF2}:
-The improvement is very large in relative terms, despite it is small in absolute terms \ref{fig:RQ2f2}.
-Req2Code and SonarQB provide an increment below 20\% in all four datasets.


\begin{figure}
\includegraphics[width=\columnwidth]{RQ2GainF2.pdf}
\caption{Percentage of F2 gain over a dummy approach.}
\label{fig:RQ2GainF2}
\end{figure}




Add another Fig 8 with results concerning Randomfoprrest only. Replace dummy with ZeroR.
Remove Figure 10.


\subsection{RQ3}
Our third and last research question (RQ3) asks ``When used in combination with other types of
metrics,  does  RCCP  improve  overall  prediction accuracy?''  

To answer this question, we construct 31 unique profiles representing each possible combination of metric groups.  We then train each of the six selected classification algorithms using each of the 31 unique profiles - producing 186 results. However prior to reporting our full results and addressing the research question we evaluate the efficacy of each classifier across each dataset and compute the number of times each classifier produces the most accurate impact predictions.  



A table reporting, for each dataset, the best combination for different sizes of combination.

\begin{figure}
\includegraphics[width=\columnwidth]{RQ3Table.pdf}
\caption{F2 achieved by groups of families of features of a specific number without a specific family (color) in accumulo.}
\label{fig:RQ3Table}
\end{figure}


A figure reporting, for each dataset, size, and group,  the gain in percentage by using the group (not as an additional group). I.e., how much the best 4 with Req2Req differes from the best 4 without Req2Req.

\begin{figure*}[!t]
 \begin{minipage}[b]{1\linewidth}
       \centering
     \includegraphics[width=.7\textwidth]{LegendRQ3.PNG}
   \end{minipage}
   \begin{minipage}[b]{.50\linewidth}
     \centering
     \includegraphics[width=1.0\textwidth]{FigRQ3Accumulo.pdf}%RQ3Accumulo2.pdf}
     \subcaption{Accumulo}\label{fig:RQ3Accumulo}
   \end{minipage}
  \begin{minipage}[b]{.50\linewidth}
     \centering
     \includegraphics[width=1.0\textwidth]{FigRQ3Ignite.pdf}%RQ3Ignite2.pdf}
     \subcaption{Ignite}\label{fig:RQ3Ignite}
   \end{minipage}   
    \begin{minipage}[b]{.50\linewidth}
     \centering
     \includegraphics[width=1.0\textwidth]{FigRQ3Isis.pdf}%RQ3Isis2.pdf}
      \subcaption{Isis}\label{lab:RQ3Isis}
   \end{minipage}     
   \begin{minipage}[b]{.50\linewidth}
     \centering
     \includegraphics[width=1.0\textwidth]{FigRQ3Tika.pdf}%RQ3Tika2.pdf}
     \subcaption{Tika}\label{lab:RQ3Tika}
   \end{minipage}  
 \caption{F2-Measure achieved by various groupings of features with a specific family of features omitted.  This graph depicts the contribution each feature family makes to achieving the maximum accuracy. For data-sets Accumulo and Ignite the greatest loss is observed when Req2Req is ommitted, and for Isis when TemporalLocality is omitted.  In Tika, the benefits of different features vary according to the number of feature groups.}
   \label{fig:AllMetrics}
\end{figure*}





==> ResultsRQ3old.tex <==
\subsection{RQ3: Which metrics support CCP?}

According to Figure \ref{fig:RQ3Statistics}, the kappa provided by the different groups of metrics is positive for all combinations but it is minor than 0.15 for all metrics groups other than temporal locality. This means that CCP outperfroms a random approach also when using only one metric group. However, when CCP uses only one group of metrics, it significantly outperforms a random approach only when using the group temporalLocality and this is true for 5 out of six classifiers.

According to Figure \ref{fig:RQ3Stat}, the best CCP classifier using all metrics statistically outperfroms the best CCP classifier using the best group (i.e., temporal locality), in all four metrics. Therefore, we can reject H30 in four out of four cases.

\begin{figure}
\includegraphics[width=\columnwidth]{RQ3.pdf}
\caption{Average accuracy of specific combination of classifier used with a specific group of metrics}
\label{fig:RQ3}
\end{figure}

\begin{figure}
\includegraphics[width=\columnwidth]{RQ3b.pdf}
\caption{Average accuracy of specific combination of classifier used with a specific group of metrics}
\label{fig:RQ3Statistics}
\end{figure}


\begin{figure}
\includegraphics[width=\columnwidth]{RQ3Box.pdf}
\caption{Box plot comparing the Kappa of the best CCP classifier when using all metrics or only the best group (i.e., temporal locality)}
\label{fig:RQ3Box}
\end{figure}

\begin{figure}
\includegraphics[width=\columnwidth]{RQ3Stat.pdf}
\caption{Kruskal-Wallis test results about the differences in accuracy between the best CCP classifier when using all metrics versus only the best group (i.e., temporal locality)}
\label{fig:RQ3Stat}
\end{figure}

\begin{figure}
\includegraphics[width=\columnwidth]{ConditionalProbability.pdf}
\caption{Conditional Probability}
\label{fig:ConditionalProbability}
\end{figure}


==> glossary.tex <==
Datasets should be replaced by "project" over the entire manuscript except for the parts where we talk about number of tickets etc. Projects reads much better than dataset to me.

Feature family: There are five families -- each one has a specific set of features. We grouped features given the concept they represent and the technology used to measure them.
Combination of features family. They have a size form 1 to 5. We could use "combination" rather than combination of features family".
Feature should never been used without "family".
When referring to F2 we should be always be clear if we mean in average among the 20 samples or for each sample.


A classifier is RandomForest or NaiveBayes.
A classifier using a specific combinations of features is a prediction model.



Feature family names:
ReqSim vs. R2RS  (requirement to requirement set)
ReqClass vs. R2C
SonarQube (SQ)
CKJM
Temporal Locality of Class Changes (TLCC)




==> old_application_to_practice.tex <==
\section{Application to Practice}
\label{sec:Practice}
In this section, we take a more anecdotal look at one example query to explore the practical implications of using our approach for automated impact prediction. For this purpose we randomly selected a new feature request from the test-set of Accumulo.  The request ACCUMULO-1009\footnote{https://issues.apache.org/jira/browse/ACCUMULO-1009} was to \emph{Support encryption over the wire} and was described as \emph{Need to support encryption between ACCUMULO clients and servers. Also need to encrypt communications between server and servers. Basically need to make it possible for users to enable SSL+thrift.}  The predictor identified 41 potentially impacted classes out of the set of 628 classes.  Of these, 17 were actually impacted, and 24 were not, leading to recall of approximately 35\% and precision of 41\%. For illustrative purposes we examine the \emph{/core/client/impl} package, which was the package containing the highest number of impacted classes.  The package includes 26 classes of which nine were actually impacted.  Our approach correctly identified four of them (\emph{TabletServerBatchWriter.java}, \emph{ServerClient.java}, \emph{TabletServerBatchReaderIterator.java}, and \emph{Writer.java}) and missed five classes (\emph{MasterClient.java}, \emph{ScannerIterator.java}, \emph{OfflineScanner.java}, \emph{ConditionalWriterImpl.java}, and \emph{ThriftTransportPool.java}).  In addition we also incorrectly identified two classes out of six as impacted (\emph{ThriftScanner.java} and \emph{ConnectorImpl.java}).

From a practical perspective this suggests that our automated impact prediction with NLP techniques can certainly not replace the human-intensive task of identifying impacted classes; however, it could potentially serve as a recommendation system suggesting additional classes for the human analyst to inspect. The state of affairs improves if the level of recommendation is raised to the package level.  At the time that ACCUMULO-1009 feature request was issued, Accumulo had 88 packages of which 27 were impacted by the change. If predictions were made for any package containing a potentially impacted class, then the impact predictor would have identified 25 packages of which 16 were actually impacted.  This would have resulted in recall of 59\% and precision of 64\%. It is well known that making predictions at the coarser-grained package level increases accuracy; however, it may be more practical to offer developers a more general, but more accurate, recommendation.

%Moreover, we believe this increased accuracy is due to chance (i.e., higher positive rations) and therefore it does not imply improved practical value \hilight{Is the final sentence necessary? } I think when the recommandation is in a more coarse-grained level, I would expect the measures would increase. I don't think that's by chance. \hilight{end}

Moreover, we expect that it would be more difficult for a developer to identify impacted classes that are isolated from other impacted classes.  In this example, the \emph{/core/client/impl} package contained nine impacted classes, three packages contained three impacted classes each, and eight packages contained two impacted classes each; however, there were fifteen impacted classes residing on their own in fifteen other distinct packages.  Our approach successfully identified 7 of these isolated classes.  In one additional case, it missed the class, but identified the package, and in the remaining 7 cases we failed to identify either the class or the package. Single class recommendations in this example would have returned precision of 87.5\% (or 100\% at the package level), with recall of 46\% (or 53\% for the package). Recommending any classes or packages that would otherwise have been missed by the developer could be very helpful in practice.

Finally we expect this approach could be particularly useful for developers that are not knowledgeable about the code base because they are recently hired or in cases where the code base is very large and the proportion of impacted class is extremely low (i.e., about 1\%) as were the case in three out of four of our analyzed projects.
